Impact of Point Spread Function Higher Moments Error on Weak Gravitational Lensing

Weak gravitational lensing is one of the most powerful tools for cosmology, while subject to challenges in quantifying subtle systematic biases. The Point Spread Function (PSF) can cause biases in weak lensing shear inference when the PSF model does not match the true PSF that is convolved with the galaxy light profile. Although the effect of PSF size and shape errors - i.e., errors in second moments - is well studied, weak lensing systematics associated with errors in higher moments of the PSF model require further investigation. The goal of our study is to estimate their potential impact for LSST weak lensing analysis. We go beyond second moments of the PSF by using image simulations to relate multiplicative bias in shear to errors in the higher moments of the PSF model. We find that the current level of errors in higher moments of the PSF model in data from the Hyper Suprime-Cam (HSC) survey can induce a $\sim 0.05 $ per cent shear bias, making this effect unimportant for ongoing surveys but relevant at the precision of upcoming surveys such as LSST.

==> processed_comments.tex <==
%\rachel{Abstracts should dive right in - not `In this project, we\dots'  Other stylistic issues: should use present tense, not future tense.  Should have 1 sentence at the start saying why this is important, like `Weak gravitational lensing cosmology is awesome, but challenges remain in quantifying subtle systematic biases associated with the impact of the PSF on the galaxy shape.'  (Not really that sentence, but something suitably motivational.)}\done \tianqing{start with PSF impact on WL}
%\rachel{Just a reminder to myself to go back over this once I've gone over the entire paper text.}
%\rachel{Should have 1 sentence at the start saying why this is important, like `Weak gravitational lensing cosmology is awesome, but challenges remain in quantifying subtle systematic biases associated with the impact of the PSF on measurements of shears from images of galaxies.'  The current motivational sentence is still way too technical.  It's a good second sentence though!  Remember that the abstract is the way to get others interested in reading your paper, and a very technical and specific first sentence may discourage those who would otherwise see your paper as relevant to their scientific interests.}\done


%\rachel{I don't see `point spread function' on the list of MNRAS keywords - \url{https://static.primary.prod.gcms.the-infra.com/static/site/mnras/document/Updated_keyword_list_Jan_2020_.pdf?node=21e8735032e6494cce9b&version=78171:e4aca8bedd490069ed08} - do you have a different and more recent version of the list?  If not, you should choose ones strictly from this list.} \tianqing{Hmm, I am not sure which one to pick other than ``gravitational lensing: weak'' \rachel{Consider ``methods: data analysis'', ``techniques: image processing'', ``cosmology: observations''}}


%\rachel{this is not how to get a tilde in front of a number.  Use $\sim$.}\done 

%\rachel{Need sentence outlining quantitative result at the end of the abstract.}\done

%%Introduce weak gravitational lensing effect and it's importance in cosmology.



    %\item The intro should mention and cite relevant past work.  So you should have some paragraph where you talk about past work understanding impacts of PSF modeling errors, including from second moments (Paulin-Henriksson, Rowe, \dots) and higher-order moments (that paper with Morgan from DESC and Lance Miller).  That paragraph should include important context, like how important are PSF modeling errors at second order in practice for current/future surveys. \done
    %\item Future surveys: WFIRST is dead; it's the Roman Space Telescope.  The citation for Rubin Observatory LSST (use that full name) should be for the overview paper by Ivezic et al 2019 and the LSST Science Book from 2009, not Tyson 2002.  You can't refer to DES and KiDS with refs to WL science papers - you need to dig up proper survey refs (their webpages will normally say).  Should mention and refer appropriately to Euclid.\done
    %\item Should not use review articles to support general statements (e.g., definition of the PSF).\done 
    %\item As a rule, you should think very carefully when giving a list of examples.  For example, you mention two seemingly random PSF modeling software packages, and three shape measurement methods ranging from antique to state-of-the-art.  This doesn't really make sense.  You can of course, in later sections, say what methods are used in this paper.  But in the intro you are setting context.  So you should (a) be clear that these are just examples drawn from the field (that's not clear for your PSF modeling examples currently) and (b) describe them in a way that makes clear why you are mentioning them -- for example, maybe you are choosing the ones on which much of the field is based, or the most recent examples, or a few very different methods to illustrate the breadth of the field. \tianqing{separate the main flow of logic from the examples.}
    %\item When defining the purpose of the paper here and elsewhere, I think you do need a caveat that the paper includes assumptions associated with ground-based PSFs (e.g., using HSC data for PSF modeling errors). \tianqing{Added the emphasis on the ground-based premise here and there and mentioned that we use HSC Y1 data}
    %\item A general figure comment: please try to use a color blind-friendly color palette (there are many out there that you can check out if you search).  You will need to find one for plots with lines, where you want a different color for each line, and another for those plots with color maps. \done
    %\item A general figure comment: if you are using color on a plot to indicate one thing, and line style to indicate another, it might not make sense to have a huge legend listing all combinations.  Rather, consider having the legend indicate one thing, and then use text on the plot to show what the line styles mean.  For example the legend on figure 3 could be significantly reduced in size this way. \done
   % \item A general figure comment: on plots with many curves, I encourage you to reconsider whether you need all the curves to make your point.  For example, you used many s\'ersic indices on figures 3 and 4.  That was a good idea when you were first working on the project, to get a sense of the level of variation.  But maybe on the final plots, you might want to space it out more?  e.g., use n=0.5, 1.5, 2.5, 3.5 (four lines) rather than six lines spaced more closely? \done
    %\item A general figure comment: The text in your figures (tick and axis labels) should be the same size as the text in the paper.  Often if is too small.  In some cases, the figure itself should be made larger or rearranged (e.g., from a 2x2 grid to a column with 4 panels) while in other cases you will need to change font size.\tianqing{I think all the font size are large enough now. Not sure if I should change the Figure 8 to one column with 4 panel?} \rachel{Figures 1-4, 6, 9 are good; the font size on figs 5, 8, 10 are still quite small.}
    %\item Do not put a space before footnotes. \done
    %\item Didn't Morgan Schmitz work on non-Gaussian PSFs in the context of Euclid?  If so, should compare to and cite his paper. \tianqing{Refer in Introduction, compare results in Section~\ref{sec:results} and Section~\ref{sec:conclusion}.}
    %\item You should try to get the figures showing up in the text around the place where they are discussed.  Right now the figures are often much later which requires a lot of flipping around.  It can take some experimentation but I would suggest working on this a bit to make the next stages of editing easier. \tianqing{The figures are pulled ahead, but still are not as closed to the text as I wish.}
    %\item When using public data or software, you should read carefully about how they wish to be acknowledged (citations, or acknowledgments at the end of the paper).  For example the HSC PDR1 cite requests a particular acknowledgment and points out a number of papers, at least some of which are relevant here and should be cited.  But please consider this for any other public software/data and check that you've acknowledged and cited them in compliance with their wishes.\tianqing{Here is what I do: I check for the following entries 1.What their websites say , and 2. What other people refer and acknowledge when they cite these things. I have checked: HSC, Galsim, Ngmix, TreeCorr, COSMOS, DESC } \rachel{Hmm. The reason I made this comment in the first place is that the HSC website (\url{https://hsc-release.mtk.nao.ac.jp/doc/index.php/acknowledging-hsc/}) requests that those who use PDR1 do 3 things, and you've only done 1 of them from what I can tell? Am I missing something?  They ask for a full acknowledgment (which you did), an acknowledgment explanation (`Based in part on\dots') which I can't find, and referencing an appropriate subset of the technical papers about the survey (which I also can't find).}\tianqing{First two items are done. For the third, I mention the main data release + pipeline and shape catalog in Section 3.4.}
    %\item \rachel{Looks like you don't have a reference to the Piff paper: \url{https://ui.adsabs.harvard.edu/abs/2020arXiv201103409J/abstract}.  Should find a good place to add it (e.g., intro, and section describing PSF modeling).}\done \rachel{Where? I don't see it in the intro or the section describing PSF modeling.} \tianqing{Sorry I made some mistakes on the changes, now it's really in the introduction}



    %\item \rachel{I recommend introducing the term `shear' early in the intro, since it gets used later on.} \tianqing{Add one sentence about shear in the first paragraph. }
    %\item \rachel{The title needs work; you cannot use acronyms in them, especially not ones you have invented yourself. You should also adopt a short title that is not `title'.} \done

    %\item \rachel{Should homogenize use of Sersic versus S\'ersic.} \done



    %\item Figure captions should really have a single sentence summarizing the key takeaways, so that people who are trying to follow the rough narrative from figures can still tell what's happening.  I think this is an important addition to make to all of your plots. \done
        %\item A general figure comment: When you have related labels on two plots, use a consistent legend (for example, don't have `regauss' versus `REGAUSS' - just call it one thing).  Also, make sure that the legend labels are clearly understandable.  For example, `mcal' should be explained in the caption as metacalibration, or relabeled.  The G/P in the legend for figure 1 also needs to be explained.  In general, look carefully at the legends and whether they make sense given the caption, or whether the caption or legend need to be modified.\done
        %\item For MNRAS, should use `Section' (capital) and `Eq.' when referring to sections and equations.  Also, need to put a tilde in between to prevent latex from splitting across lines, i.e., `Section~\ref{repofhome}' rather than `Section \ref{repofhome}'.  (Look at the latex to see the difference.)\done
        %\item I notice you sometimes use S\'ersic and sometimes S\`ersic.  It should only be the first one, not the second one - should fix to be consistent.  If you have trouble remembering, you could also define a latex macro for it. \tianqing{Thanks for pointing out}
        %\item Correct me if I'm wrong, but I don't see an explicit statement early on that by using round PSFs and only considering radial kurtosis, by definition we only need to explore multiplicative bias -- and future work will need to consider non-round PSFs and other moments, which could generate additive biases.  Was this said anywhere (e.g., in the introduction when explaining the scope of the paper) or should it be added?  It's a pretty key methodological simplification.\tianqing{I add a sentence in the introduction to point out this limitation and a paragraph in Section 3.3.2 talk about this.}

        %\item Watch out for the difference between `e.g.' and `i.e.'.  `i.e.' is a way to refer to a definition or equivalent terminology, while `e.g.' is for examples.  So if you want to cite a paper that is an example of how some method is applied, that is a place for `e.g.', not `i.e.'. \done


    %\item Do I use ``Higher order moments'' or ``Higher moments''? \rachel{Hmm. I guess, now that you mention it, ``higher moments'' is probably more standard usage.}



%\rachel{note this previously said only shape was modified, which is incorrect} 


  %\rachel{I recommend citing the well-regarded review of dark energy led by David Weinberg about 5 years ago - it has a nice comparison of methods including weak lensing.} \done 


%\rachel{may I ask where you are getting your bibtex?  This reference is incorrect - see ADS, it should have the survey collaboration as the first author, not Abbott: \url{https://ui.adsabs.harvard.edu/abs/2016MNRAS.460.1270D/exportcitation}}\tianqing{Ah, I went to inspireHEP for the citation. Next time I will use ADS in priority. } \done, 



%\rachel{no - this is not the correct reference for Euclid. I realize it can be hard to figure out the right one, but one tip I have is to look at where it's published and what is its content: this is a 3-page conference proceeding.  Any official survey reference is going to have more content and will likely either be in a journal or just a design report on arxiv.  For Euclid, use this: \url{https://arxiv.org/abs/1110.3193}}\done 

%\rachel{When you have a sentence with a long list in it, you should put the core content up front.  In this example, I would suggest saying `The requirements on control of systematic uncertainties in weak lensing measurements become tighter as the statistical errors decrease to sub-percent levels, starting from Stage III surveys \dots and moving to Stage IV surveys \dots.  It's hard to read a very long list and then focus on and comprehend the content that comes after, so better to make the point first and end with the list.}\done 

%%Introduce PSF and it's connection with weak lensing.

%\rachel{The next sentence is incorrect in a few ways.  First of all, for ground-based telescopes, the atmosphere and optical PSF convolution occurs before the light reaches the focal plane.  Second, the sentence structure seems to imply that there is no PSF for space telescopes.  I don't really understand what point is being made - can you clarify?  (Or, perhaps the sentence is not needed?)} \tianqing{I was trying to say that PSF will change the shape and size of the observed galaxy, but this is pretty obvious so maybe it can be removed.} 

% Note, it's Piff, not PIFF.

%\rachel{I edited to reduce the number of methods mentioned.  It's hard to justify calling out 4 different methods in the intro; generally you should either aim for completeness, or the most recent examples, or some other well-defined scheme rather than four that seem somewhat random.} \tianqing{I add PIFF here}

%\rachel{You should propagate this change elsewhere: it's `true PSF', not `truth PSF'.} \done 

%\rachel{Use them to do what?  Remember the paper has to be accessible; you can't expect readers to fill in the dots.}\done 

%\rachel{Note: it's not one of the main uncertainties in weak lensing overall, just in shear inference.} 

%\rachel{`HSC Y1' is not a phrase that is used by the HSC survey - need to either define it, or avoid}\tianqing{Change all to ``first year shear catalog" and ``HSC public data release 1 (PDR1)'', or, simply say ``HSC''} 

%\rachel{Note edit here: after the initial definition of Rubin Observatory LSST, can just call it LSST throughout.}\done

%Scope of this work, and the arrangement of this paper

%\rachel{you've never defined this acronym} \tianqing{I am actually not sure if I should use ``Higher order moments'' or simply ``higher moments''}

%\rachel{broken ref}\done 

%\rachel{Outline should be the start of a new paragraph.}\done 

%\rachel{Note the need for parallel structure: it's not `section X does Y' but rather `In section X, we do Y'. (This is just an explanation of my edits - you don't need to do anything else here.)} 

 % \rachel{This is all true but too vague.  You should make it clear that these subsections are about the background of weak lensing, PSF, and galaxy shape measurement.} \done


%\rachel{As a rule, you can only use a review as the reference for a general/foundational statement if you say explicitly `for a review, see X'.  Otherwise people will say `there are lots of papers on this, many of them earlier, so why are you doing this?'}\done

%\rachel{Somewhere in this section you need to indicate that the convergence/shear is related to the gravitational potential, and that's how the connection to structure growth and cosmological parameters comes in.  Otherwise the first paragraph and the rest of the section are totally disconnected.}\done

%\rachel{That review is about systematics, but I think in this section a review about the science is more appropriate.  For example, the Kilbinger review would be a good choice.}\done 

%\rachel{watch out for quote marks in latex}\done 

%\tianqing{I think it's more natural to bring up the linear transformation first, then talk about shear and convergence, the measurement of shear etc. } \rachel{Sure, seems fine.}

%\rachel{I'm not familiar with this term `locally-homogeneous' when applied to linear transformations; can you clarify or point me to a reference using this terminology?}

%\rachel{hmmm, the equation below appears to be the opposite of what I normally see in the literature; are you sure they are not swapped?} \tianqing{You are right, I change the order. }

%\rachel{technically it's a spin-2 quantity in 2D (vector means something a little different)} \done

% \rachel{is it necessary to give this example only for a round galaxy?  You could simply say that the convergence changes the galaxy size (regardless of its shape), while the shear induces a change in shape - and then give the `circle to ellipse' example.}\done,

%\rachel{Missing background here: what does it mean for the shear to be an imaginary number?  What, physically, is the convergence?  Can you make some statement about what this matrix actually does to a circle or an ellipse?} 

%\rachel{superscript letter `o' is not how to indicate degrees - use the `$\circ$' command}\done

%The former one has a lower signal-to-noise ratio \citep{2001PhR...340..291B, 2010MNRAS.401.2093V}, which has driven an emphasis on measuring shear.
%% RM: I commented the above sentence out.  S/N is not always the primary issue here - it's the lack of a good null for magnification, and measurement challenges associated with it.
%\rachel{This is a bit confusing.  Suggested rewrite: `Measuring the convergence directly would generally require assumptions about the pre-lensing galaxy sizes, whereas measurement of shear relies on the fact that galaxy shapes are generally presumed to be randomly oriented in the absence of a coherent weak lensing shear signal. That has driven an emphasis on measuring shear.'  (and insert appropriate references, plus a footnote that intrinsic alignments breaks this assumption - also with references)  }\done
%We measure the shear $\gamma$ by taking the average of the shape of the galaxies. \rachel{That is true in the case that there is a constant $\gamma$ in some region, which does not describe all scenarios in shear measurement - so, some clarification is needed.} Although each galaxy in the sky has its own intrinsic shape, we can measure the weak lensing shear based on the assumption that the intrinsic shapes are randomly oriented, as long as the intrinsic alignments \rachel{This is a term you have not defined.  Your choice is to either define it, or to {\em not} define it, in which case you should simply describe what you mean in less jargony terms.} are handled in the modeling process.
%\tianqing{I find the paragraph commented above really bad, so I just delete it. }
%Since it is hard to make assumption to the pre-lensing size distribution of the galaxies, it is common to write 

%\rachel{This is from numerous earlier theory papers, so I would not cite my review - you should either not cite because it's ubiquitous usage, or cite an early theory paper} \tianqing{I change it to Scott's book.}. 

%\rachel{Should use math mode inside of the text where appropriate, e.g., $(x,y)$ rather than (x,y).}\done
%\rachel{For reference, I did some compression of the text around here.  Generally one should not repeat quite so much background material from the introduction.}

%\rachel{There are some inconsistencies in these references that I suggest you homogenize.  In particular, I recommend citing only shape catalog papers, not cosmic shear measurement.  So you can keep the HSC catalog paper, but I recommend citing the latest DES and KiDS catalog papers as well: \url{https://ui.adsabs.harvard.edu/abs/2018MNRAS.481.1149Z/abstract} and \url{https://ui.adsabs.harvard.edu/abs/2020arXiv200701845G/abstract}.} 

%\rachel{And here is a good place to refer to the cosmic shear or 3x2pt analysis papers, one each from HSC, DES, KiDS}. %\rachel{could refer to any review of WL such as Kilbinger, or alternatively, to the shape catalog papers for HSC/DES/KiDS} \done 

%The transformation matrix above is still a mix of magnification of size and brightness and the stretch of the shape, but we can further separate the magnification and distortion by defining the reduced shear $g_i = \gamma_i/(1-\kappa)$. The transformation then becomes

%\begin{equation}
%\begin{pmatrix}
%x'\\
%y'
%\end{pmatrix} = (1-\kappa)
%\begin{pmatrix}
%1-g_1 & -g_2  \\
%-g_2 &1+g_1
%\end{pmatrix}
%\begin{pmatrix}
%x\\
%y
%\end{pmatrix}. 
%\end{equation}

%\rachel{I'm finding this discussion below to be mixing terms in a somewhat confusing way, but also, it's not clear to me why you want to treat systematic uncertainty differently (and later in the section) compared to statistical uncertainty.  My recommendation: in a single paragraph, introduce the concept of statistical uncertainty (don't use `error' since it is ambiguous), systematic bias, and systematic uncertainty.  This will require you to restructure the discussion below in a few ways.  I've not done any thorough editing } \tianqing{The following paragraphs are rewritten. }

%\rachel{Equation is a bit odd - the left hand side is a standard deviation but the right-hand side is a variance.} \tianqing{Added square root}

%\rachel{inconsistency: $n$ versus $N$}\done \rachel{You already defined $N$ above the equation, so you don't need to define it again below the equation}\done.

% \rachel{The next sentence seems to duplicate what you said above - do you really want to repeat it?}\tianqing{I though before I am talking about shape noise, and after I am talking about cosmic variance.} 

%\rachel{You should find a paper to reference regarding sources of statistical uncertainty - e.g.\ Sukhdeep's paper about covariances might have some foundational ones you can point at.}\done

%\rachel{citation!}\done. 


%There are two different kinds of error in the shear signal: statistical uncertainty (or variance) and systematic uncertainty, where the former is manifested by the width of the distribution of data, the latter one is by the shift from the truth due to the mis-modeling of the systematic biases. 
 
%The statistical error of weak lensing can be considered as two parts: the shape noise of the galaxies and the cosmic variance. The randomness of the intrinsic shape of the galaxies causes the shape noise $\sigma_{\langle \gamma \rangle}$. %\rachel{Need to briefly mention intrinsic alignments as violating that assumption, but being dealt with at the modeling stage.} %\done 
%\rachel{This equation assumes one is measuring shear by just averaging a bunch of galaxy shapes, so it doesn't apply to some of the measurements you mentioned such as two-point correlations.  Some clarification is needed. (Or a more general equation, or no equation at all.)}  Cosmic variance caused by the large-scale structure of the Universe is also a source of statistical error for weak lensing observations. As the weak lensing surveys grow deeper and wider in area, the cosmic variance becomes more important than the shape noise as the main source of statistical uncertainty in weak lensing. \rachel{Reference needed!} %\rachel{Mention cosmic variance, which is more important than shape noise for large surveys.} \done 

%\rachel{Need to elaborate on that point.  You're assuming (but need to state) that one does not want systematic biases or uncertainties to dominate over the statistical error. I would, further, briefly define systematic bias versus uncertainty, and make sure to use the terms consistently throughout the paper.} \done \rachel{I don't see where you have made the distinction between systematic biases versus systematic uncertainties?} \tianqing{elaborated the connection between systematic bias and systematic uncertainty.  }

%\rachel{its systematics?  Or systematics induced when one does not model it effectively?}

%\rachel{The phrasing of some of this discussion is a bit odd - I suggest reading a few papers about PSFs and looking for key phrases to use.} Point Spread Function (PSF) is a class of function that describes how a point source is distributed on a 2-D plane after a certain optical process. For a ground based telescope like LSST, the main source of PSF comes from the atmosphere above the telescope, and the optical structure before the light reaches the focal plane. Therefore, we can divide the  PSF into two parts: atmospheric PSF and optical PSF. \rachel{You should clarify that you're talking about the {\em effective} PSF, i.e., including convolution with the pixel response function.}

%\rachel{Next two paragraphs particularly need references.}

%The atmospheric PSF describes how atmospheric turbulence smears the light from the galaxy over the period of exposure. A common theory that predicts atmospheric PSF is called the von Karman turbulence model, with two parameters: the Full Width of Half Maximum (FWHM) and outer scale. Setting the outer scale to infinity, the von Karman model reduce to the Kolmogorov model \rachel{which you haven't defined}.  Typically, the best FWHM of atmospheric seeing for an outstanding site is around 0.5 arcsec. 

%The Optical PSF is introduced by the telescope diffraction effect, defocus, comas and other imperfection of the optical system. The optical PSF is specific to telescope, and is more significant for space-telescope, since there is no atmospheric part for the space telescope. 

%PSF will wipe off the detail of the galaxy that are smaller than the PSF and most importantly dilate the shape of the galaxy, which will affect the weak lensing measurement. As a results, we need to model the PSF, which will be detailed in the section \ref{psfmodel}. With the PSF model, we can then recover the true shape of the galaxy with the shape measurement methods that will be introduce in depth in section \ref{shapemeasurement}. \rachel{More precision needed especially in next sentence.} However, the PSF model is hardly exact the same as the true PSF, and will be introducing systematic error to the weak lensing shear.


%\tianqing{I combine the "PSF" section and the "PSF modeling" section as what it is now. I also skip the background for the physical nature of PSF: since we are using the empirical approach, introducing PSF from the physical point of view does not really make sense to me.}

%\rachel{The first two paragraphs of this section are notably lacking references.} \tianqing{Add references.}
%\rachel{I recommend editing the first two sentences of this paragraph for consistency with the description of the PSF in the introduction.  There is a certain amount of non-standard use of terminology here that I fixed in the intro:}\done

%note not all WL measurements use CCDs - some use NIR detectors - so `detector' is more inclusive language

%\rachel{here would be a good place to cite metacal and BFD papers}\done 

%\rachel{I inserted this sentence to make very explicit the connection between WL shear inference and PSF models, which ties into the next paragraph.}\tianqing{Noted}

%The effective PSF modifies the observed shape of the ga laxy, which \rachel{here `which' modifies `observed shape' - I think you want to refer back to the pre-PSF shape?  May need to modify the logic of the sentence} can be measured by shape measurement methods developed such as KSB \citep{Kaiser:1994jb} and re-Gaussianization \citep{Hirata:2003cv} \rachel{this is true, but it's a case where a WL expert would likely be perplexed at the fact that you mentioned these two out of the many methods that exist (why these two?  why only two very old ones?  etc.).  My recommendation is to refer to the GREAT3 results paper for a collection of methods as of 2015, and to the KiDS, HSC, and DES catalog papers for what has been used recently in practice.  At some point you will have to specify which methods you use in this paper, but that's in the methods section, not here.}, given the PSF model at the position of the galaxy. Incorrect PSF modeling means that the wrong PSF will be used in the shape measurement process; this results in systematic biases in the shape and weak lensing shear estimation process \citep{PaulinHenriksson:2007mw, 2010MNRAS.404..350R, 2013MNRAS.429..661M }. \rachel{Whenever you have a list of references in one place, you should put them in time order.}

%\rachel{cite relevant papers from DES, KiDS, HSC analysis}\done, 

%\rachel{Should comment on hybrid approaches, wavefront modeling, etc.  Should also comment on how PSF modeling is done in cases where there are multiple images at a given point on the sky.} \tianqing{The only example I found for this is Roodman's paper in 2014 (mentioned in your review) but I don't know how to access it..} \rachel{I suggest asking Josh Meyers for a good reference for wavefront modeling approaches.  Regarding coaddition, your above text could use some adjustment -- it is not necessarily the case that a coadd has a well-defined PSFs.  It depends entirely on how the coadd is generated.}\tianqing{What I was saying there is specifically about HSC pipeline, I have fixed it.}

%\rachel{Check MNRAS author guidelines - I'm pretty sure they require small caps rather than italics for software}\tianqing{That's right, I have fix all software/package name}

% turns out CMOS detectors also have brighter-fatter, so it's not just CCDs

%\tianqing{Mentioned detector effect here. } \rachel{Need to elaborate slightly and provide references.} \done  

%\rachel{You should probably cite a paper here.  For example, the Bosch et al HSC pipeline paper is a good one.  I believe all tests except for one using the stacked image of residuals rely on second moments.}\done 

%\rachel{you might consider `light intensity profile' or something more specific than `distribution'.  To be clear, your equation makes sense for a general distribution, but some of the later terminology (like referring to the normalization factor as a `flux') is specific to how we talk about light intensity profiles.  If you make this change, it will also require some changes in the text below the equation}\done 

%
%\rachel{Another important conceptual point is that some detector effects that are not part of the PSF (i.e., they are not mathematically convolutions) may induce PSF modeling errors because their effect on bright stars may not be perfectly corrected.  So PSF modeling errors can also be due to detector effects.}
%
%\rachel{In an equation, you shouldn't have $1/F^{(0)}$ before another term -- only divide by things at the end. Or, use the `frac' command to make a fraction.}\done
%\rachel{Do you want to introduce a weight function into the integral and comment on the various cases of unweighted and weighted moments?  It seems relevant.}\done
%
%\rachel{When including terms or partial terms in subscripts/superscripts, such as `cen' which is short for centroid, or `gal' or `PSF', should put it in a text box.}\done
%\rachel{I fixed this here, but for reference: when you are explaining an equation, you should not start a new paragraph.  The explanation belongs to the same paragraph.}\tianqing{Noted.} 

%\rachel{Defined using the same weight factor?}\tianqing{Further specified} 

%\rachel{again comment on use of weight in centroid determination}\done.

%\rachel{Consider defining the trace and using it here.  Also consider explaining the relationship to the semi-major and semi-minor axis lengths, to provide some more physical understanding of what these equations do.} \done


%\rachel{check: is this per-galaxy ellipticity bias?  Or ensemble shear bias?  Also, is this the same $e$ definition as you used previously?} \tianqing{This is per-galaxy ellipticity. In the paper, all the $e$s are un-weighted, however, I have confirm that this formula works for weighted moment as well.} 

%\rachel{use `left(' and `right)' commands when putting parenthesis around a fraction}\done

 %\rachel{should clarify whether it's the pre-seeing radius of the galaxy, or radius of the PSF-convolved galaxy image} \done. 

%\rachel{don't hard-code equation numbers!  Use `Eq.~\eqref{eq:desys}' with a reference}\done 

%\rachel{Here is a good place for references that illustrate the process of setting requirements.} \done %\rachel{The term you should introduce is `requirement', not restriction.} \done

%\rachel{careful in use of citep versus cite} \tianqing{I didn't know citep means cite with parentheses} 

%\rachel{The rest of the paragraph seems incorrect to me.  The Rowe+ paper define $\rho_1$ and $\rho_2$, which involve PSF model {\em shape} errors (only), not size errors.  The Jarvis+ paper defines $\rho_3$ through $\rho_5$ which include combinations of PSF model size and shape errors.  In both cases, they lead to additive biases.  I suggest looking this over again and correcting the rest of the paragraph.} \tianqing{Re-written} 

%\rachel{Should give later examples of this being done in cosmological weak lensing analyses.}\done

%\rachel{Here is a good place to comment explicitly on biases and uncertainties - i.e., well-quantified PSF modeling errors lead to WL shear biases that can be removed, while systematic uncertainties in PSF modeling errors lead to WL shear biases that must be marginalized over.}\tianqing{Should I give examples?}

% is overlooking %\rachel{careful - that's not what this word means - overseeing means that you are carefully watching something, while an oversight is something you are neglecting, because English is a stupid language} \tianqing{Ah, I meant overlook not oversee, ouch}

%\rachel{need more words here like `how accurately the higher order moments of the PSF are modeled'}.\done 

%\rachel{broken ref}\done 

%\rachel{please confirm this last phrase I've added - I think that's what they did, and it's necessary to explain why additional biases were found.  Do I recall correctly that they used a realistic Euclid PSF model but did not try to diagnose more specifically which aspects of the PSF led to the additional biases?  I think that might explain your next sentence, but please clarify.}\tianqing{I think it's right, their PSF model is very realistic. }.\done 

%\rachel{Should search places where the `HOME' acronym is used and replace if you decide to call this something different.} 


%\rachel{Need to fix - always use present tense throughout the paper.}\done
%\rachel{This paragraph seems out of place in the background section.  Might it go into the methods section or elsewhere?  Note that I've not edited it in detail (it does need some editing if retained) but I wanted to wait until it had a more natural place in the paper.} \tianqing{Right, it is half repetitive words about what this paper is (that we already say in Introduction) and half conclusion we reach at the end, so it shouldn't be here nor in Method section. }
%The HME serves as an additional systematics induced by the PSF model. Therefore, this is more important for a survey with an already tighten error budget. For the LSST, the 10 year requirement for PSF model size error is  $\text{sub-}0.1\%$ \citep{2020MNRAS.496.5017G}\rachel{Citation needed!}\done, which means the shear bias induced by HME of PSF model should also be controlled at the same level.  %\rachel{Should give quantitative background: how tight are the error budgets for shear calibration for LSST, Euclid and what does that mean in terms of PSF size? This set the stage that with sub-percent precision needed in PSF size, it's logical to investigate higher order moment errors}\done


%\subsection{PSF modeling algorithms}
%\label{psfmodel}

%%Need reading. 
%Modern surveys utilize a specific set of stars called PSF stars to estimate the local PSF and estimate the PSF at the galaxy by fitting a position-dependent model though the exposure or focal plane. The selected PSF stars are bright enough to ensure signal-to-noise ratio but not too bright so that some pixels saturate and therefore misrepresent the true PSF. \rachel{Need to be more quantitative (typical S/N and density) and cite survye papers for more details of modern PSF modeling, e.g., Bosch et al HSC paper.}


%Describe overall approach: different stages of the analysis.  Subsections then describe the tools used for those analysis stages.

%\rachel{Use present tense, not future, throughout the paper.  `In this section, we describe\dots' (there are a few places where this is relevant throughout this section - you can do a search for the word `will' to find them).} \tianqing{There are 48 ``will"s} \done

%\rachel{The next sentences are a little cryptic, in the sense that the subsections do not clearly indicate an obvious image simulation versus real data thread.  Sections 3.1 and 3.3 are more general methodology that is applicable to both.  Might you consider some reorganization?  For example, perhaps you could move section 3.3 before 3.2, so that the general aspects of the methodology are first, then image simulations, then data?  That might result in some changes in the intro to this section, as well.} \tianqing{I change the order and re-write this paragraph} \rachel{The next sentences are now pretty clear.  But I was wondering if they are needed?  The paragraph after this walks through what each subsection and explains how the threads relate.  So maybe the rest of this paragraph is not needed?}\tianqing{Sure, I just stick the first sentence to the second paragraph.} We first introduce the general methodology of our experiment: defining higher moments of PSF and shear measurement method. Then, we introduce the two approaches we take toward this problem: image simulation and real data inspection. Ultimately we combine the two approaches to predict the impact on shear systematics caused by HME. 

%\rachel{Say {\em why} you are using real data and how does that relate to the image simulation thread, to give the reader a road map to understand how all these subsections relate to each other.} \done

%To study the level of impact caused by higher moments of the PSF modeling, we must first define the higher moments of the light profile. 

% and modified for the image simulation.

%When we modify the model PSF by these methods, we are changing all the raidal higher moments. 

%\rachel{how?  your own code, or GalSim?}\done 

%\rachel{First reference to this code in the methods section needs a citation and URL to the repo.}\done. 

%\rachel{Need to define $r$ and $\omega(x)$; and I think $x$ should be $\mathbf{x}$.  Also, here you used $I(x)$ but in equation 3 you used $f(x)$, and you might want to consider unifying the notation.}\tianqing{No more $I(x)$}


%\rachel{should this be $r=|\mathbf{x}|$ for consistency of notation?}\done 

%\rachel{The next sentence is over-specifying: we don't only define the kurtosis bias that way for modified effective PSFs versus originals -- we use this definition for real data, e.g., for the PSF model and star images without modification.  I suggest rewriting the sentence and equation to make it more general.}\done 

%\rachel{All the hats here are in the wrong place.  They should be on the $\rho$ part of the $\rho^{(4)}$.}\done
%\rachel{In general, equations that are not inline should use actual fractions rather than `/'.}\done

%\rachel{how did you decide it was small enough?}\tianqing{such that the value of kurtosis converge to the second decimal.} \rachel{You should say that in the text or caption.  In general, saying `it converged' isn't very meaningful or reproducible without a quantitative statement of how you decided it was converged.}\done

%\rachel{What's the purpose of the first column?  Do you ever use it?  If not, I would remove it.}\done

%\rachel{We don't want to focus too much on re-Gaussianization.  I would simply state that we are using the change in the 4th moment as an indicator, while acknowleding that other moments have been modified.} \done

%%Need more reading

%\rachel{Consider modifying the title.  Metacalibration in particular is a {\em shear inference} method, not a shape measurement method - it's really defined for an ensemble.}\tianqing{change to ``shape and shear measurement"}

%\rachel{I edited/commented down to here.}

%\rachel{I think you should make this a separate subsection.  It's not a part of the image simulation process; rather, it's part of your analysis.} \done

%\rachel{This section has no references, no mention of what shape measurement method is being used, and no mention of the specific implementation/software.  This all needs to be fixed.  Perhaps move section 2.3 material into here, instead of having two separate sections on this?  Or, call back explicitly to that section for references, but you still need to use names of algorithms etc.} \done

%\rachel{The subject is definitely {\em not} agnostic to the shape measurement method.  In detail, the impact of HME will definitely depend on the method, though we will try to assess the degree of sensitivity by using multiple methods.  Should rephrase/rearticulate this point.}\done
%\rachel{I suggest opening with a preamble that states that you use a few methods of ensemble shear inference, some of which involve averaging per-object shape estimates.  For this reason, you will investigate  galaxy shape biases as a step towards the real target, biases in inferred WL shears.  This would involve editing the first couple of sentences of this paragraph:}\done

%\rachel{PSF calibration is not a phrase.  I think you mean PSF modeling and then shape measurement while correcting for the PSF}\done

%The last step of the simulation is to measure the shape of a single galaxy, or the shear of the 90-degree pair or an ensemble of galaxies, calibrated by the slightly tweaked PSF model. To start with, we convolve the galaxy with the true PSF, then convolve with the pixel to generate a final image that the shape measurement method observes. The PSF model is also convolved with the same pixel function to generate a PSF image, know as the effective PSF. \rachel{HEre's another place that would be simplified by defining the standard term `effective PSF' early on, and using it consistently throughout the paper.}\done

%\rachel{Here again you should unify the notation -- consider whether this should be $e$ or $e$.}\done  \rachel{Also, I suggest using hats consistently for estimated quantities, i.e., the estimated shape or shear are $\hat{e}$ and $\hat{g}$ to distinguish them from the true values.  This is a change that I suggest you make throughout this section.} \tianqing{Yes, I should use hat rather than subscripts such as ``model" and ``truth"} \rachel{Finally, I don't see $\delta e$ or $\delta g$ referred to later in the paper, in either the text or figures, so is this statement out of date or should the notation be introduced more consistently later on?}\tianqing{They show up in a lot of plots, on the y-axis label. It is my bad though, since the y-axis label was dis-organized. Now they are fixed. }

%\rachel{I suggest you consider turning this paragraph into equations.  But for now I've at least introduced some notation.}\done 

%\rachel{General comment: when you have an estimated quantity denoted with a hat, and you put a subscript, you need to put the hat only on the quantity and not on the subscript - i.e., it should be $\hat{e}_{90}$, not $\hat{e_{90}}$ - look at the compiled PDF and you will see how the hat is correctly in place for one of these and totally off for the other.  So that should be fixed in the above and elsewhere.}\done  
%\rachel{But another point: here you seem to be implying that shape and shear are vector quantities (using mathbf for them).  They aren't really vectors, rather they are spin 2 quantities, so I suggest just using regular math mode.  You could say these equations are defined component-wise for each component.}\done

%\rachel{Specify that you are using Erin Sheldon's implementation in the ngmix package, with link, and whatever references he asks people to make when using his code.} \done \rachel{Sorry, I don't see a link to his code - where is it?}\tianqing{put the URL}

%\rachel{Notation: sometimes you're using $g$, sometimes $\gamma$ - is this intentional?} \tianqing{I used $\gamma$ to stay consistent with the referred paper. I probably should stay consistent with my own notation: $\gamma$ as shear and $g$ as the reduced shear.  } \rachel{That's right.  Section 2.1 would be a good place to introduce this notation and state you'll use it consistently throughout (and then fix this to be consistent).  But currently I don't see reduced shear defined in section 2.1.}\tianqing{I've add definition to reduced shear $g_i$ in Section 2.1, and point out that since we are not considering magnification, the reduced shear is the same as shear.}

%\rachel{Should some of the $e$'s and $g$'s below be $\hat{e}$'s and $\hat{g}$'s?}\tianqing{Yes}

%\rachel{Again, no fractions in inline equations.  Just do $\partial e / \partial \gamma$.}\done 

%\rachel{You seem to be avoiding talking about the fact that this is really a matrix - is this deliberate?} \tianqing{Change to metric rhetoric.} \rachel{Sorry, do you really mean `metric'?  I think it's just a standard matrix, as described for example in the Huff \& Sheldon metacalibration paper.}\tianqing{For some reason I thought ``metric'' is the adjective of ``metrix''... My bad! I have fixed it.} 

%\rachel{it's not the true shear - it's our shear estimate for the ensemble, right?}\tianqing{Yes} 

%\rachel{Is there a reason not to make this a proper fraction?}\tianqing{Because it is ``multiply by the inverse of the matrix response'' rather than ``divide by the matrix response'', one can not divide something by a matrix?}

%\rachel{Edited up to here.}

%\rachel{Are they the {\em main} objects you simulate?  Or the only ones?  `Main' makes it seem like you do sometimes simulate other things, just not too often.}\tianqing{Sure, I've made it clear} %\rachel{This reads like 3 steps: generated galaxy profiles, PSF profiles, and shape measurement?  But shape measurement is not in this subsection, so maybe just don't mention it?}.\done 

%\rachel{I'm concerned that the table is a little complex, with 5 different options.  For a casual reader, it would be valuable to provide a clear roadmap to it -- for example this could be a final subsubsection clarifying the purpose of each of the five simulation sets, and giving a direct reference to where the results will be shown.  You would also benefit from more explicitly referring to it within the text; a table can be a powerful organizational tool, and leaving it completely unreferenced within the subsection text is a lost opportunity.  For example, you could label each simulation set with a number that you refer to within the text (for example: `Using simulation set 1 from Table 2, we test XYZ.').} \rachel{Also, note that the table does not include parameters for all simulations, as the previous sentence implies.  I think it's OK to limit the table to describe the single-galaxy simulations, but you should make sure the description of the table in the text is clear about that.}\tianqing{I clean up the table a bit: remove the shape measurement column, and add the index column. I add a subsection 3.3.3 to describe the road map of our simulation, including what is in Table 2 + COSMOS catalog. I link the description to the results section and, in the results section, refer back to the table.}

%\rachel{In this introduction to the section, I suggest giving a high-level description of the simulations.  Many people use many types of simulations for different purposes, and there is a lot of background you have not provided: for example, that these are {\em postage stamp} images of non-blended galaxies, with infinite S/N.  I think you have a common pixel scale for all images, which you should also mention.  In short, I encourage you to think critically about what aspects of your simulation setup you have not described, and put it here before you start talking about the galaxy profiles.}\done

%The shear or bias of the ensemble due to kurtosis error in the PSF model is the difference between the estimate shear using true PSF: $\langle \hat{g}_{\text{true PSF}} \rangle$,  and the biased estimated shear measured by the model PSF: $\langle \hat{g}  \rangle$. \rachel{Careful - with the subscript on $\gamma$, it looks like you're talking about the true weak lensing shear.  I think you want to indicate the PSF used for measurement in some different way.} This shear bias can be related to the true input shear and decomposed in a linear model with additive and multiplicative bias.  However, since the PSF \rachel{Should this be PSFs?}\tianqing{Yes} used in this work are round, there is no additive term in practice. 

%\rachel{I think this is a little confusing.  Why not just a comma, which is typically used to separate the items in a list of distinct items?}\done 

%\rachel{I think using a hyphen -- would be more standard.}\ 

% \rachel{OK, but might it be more to the point to say that the `kurtosis error' is given by equation 6?}. 

%\rachel{Need to turn this into a sentence.}\done

%\rachel{Try to use consistent units where possible - e.g., one cannot compare $\sigma$ and $R_h$, so perhaps use $R_h$ for all profiles?  Consider giving each row a label, so that the results can refer to the specific row?  Define kurtosis with a pointer to the equation, since most people will not realize you may be talking about a radially-weighted quantity.}\tianqing{About unifying the unit for the scale factor: If we use $R_h$, we will need to change the quantity used in the plots, if we use sigma, we will have to rerun the S\'ersic experiments because we use $R_h$ to define the size of S\'ersic profile.} %\rachel{Should `Kurtosis Error' in the table and caption be `Fractional Kurtosis Bias'?} \tianqing{Correct.}

%\rachel{Need to give numbers at some point for the sims.  Perhaps you could tabulate galaxy, PSF, etc. info into a table.} \tianqing{Added a table}

%For all the galaxy images, we first make a round galaxy, and distort the profile to make an elliptical galaxy. \rachel{I thought some of your experiments include galaxies that are not round, i.e. you are directly drawing only a galaxy with some shape rather than drawing a round galaxy that you distort?}\tianqing{Ah, I meant to describe the way I draw elliptical galaxies.} \rachel{Do you mean that you apply galsim.Shear() to the GSObjects?  If so, I do not think you need to describe it like this.  I think this could lead to some confusion about actually drawing a round galaxy and then modifying it.  So I actually think this sentence could be omitted.} %\rachel{At what point in this list do you go from measuring shape of a single galaxy to measuring shear from an ensemble?  It's not quite clear.} \tianqing{Add the specification}

%\rachel{Previously, between equations 3 and 4, you defined an ellipticity $e$.  If this is meant to be the same quantity, you should use a consistent symbol here.}\tianqing{Yes.} 

%\rachel{need citation for claim!}\done

%\rachel{Don't hard-code references.}\done 

%\rachel{I suggest not using $e$ here, given that $e$ means something else in your paper.  Rather, you can use $\exp{-b (R/R_h)^{1/n}}$.}\done

%\rachel{You haven't said what $b$ is.}\done %\rachel{What you haven't said, I think, is that you also carry out some simple simulations with fixed S\'ersic parameters?} \tianqing{I don't understand this.} \rachel{Here is what I mean: you introduce the S\'ersic profile as a more realistic light profile.  Then you simply move on to say you use the COSMOS S\'ersic fits.  But that doesn't describe your workflow.  You {\em first} did controlled tests with individual galaxies of a particular S\'ersic index and size, for example in figure 5, before proceeding to the COSMOS galaxies.  So you should say that here.}\done

%The S\'ersic profile is a commonly used model to describe the galaxy profile.

%\rachel{say what band}\tianqing{Change for all} 
%\rachel{Technically it's F814W magnitude}

%\rachel{Clarify: is it a half-light radius or flux radius?  Those differ: one is pre-PSF convolution and the other is post-convolution.}  \tianqing{Hopefully it's clearer now. It's the flux radius, but the HST PSF is small, yes?} \rachel{True, but should still check how much this matters (I think we discussed this) - it can be more important than you'd guess.}\done \rachel{Where is it done?}\tianqing{I add a clarification and the size of the optical PSF here.}

%\rachel{What is `realistic parametric distribution' meant to convey?}\tianqing{It means we want more a realistic galaxy sample set.} \rachel{I suggest rephrasing to `galaxies with a realistic distribution of size, shape, and S\'ersic indices'}\done,

%\rachel{The implementation within GalSim is not described on this wiki - only the datasets and how to get them are described there.  Perhaps we should move the footnote so it is more clearly associated with the sample of galaxies?} \tianqing{I don't know if the current position of the footnote is what you are asking for}.

%\rachel{put the key COSMOS citations}\done 

% \rachel{What is intended by `general S\'ersic fitting'?  Do you mean that you use fits to a single S\'ersic profile even when fits to a double S\'ersic are statistically preferred?} \tianqing{Yes, I think the catalog always have Sersic fitting, and sometimes bulge-and-disk fitting. I always take the Sersic fitting.} \rachel{Right.  But to be clear, people will generally say that bulge+disk is also Sersic fitting (it's just fitting two of them).  For clarity, I suggest referring to these as single Sersic fits rather than just Sersic fits.}\done in the catalog 

%\rachel{Aren't you using \code{COSMOSCatalog}, which knows how to reconstruct the S\'ersic profiles, unlike \code{RealGalaxy}?}\tianqing{Right.}

%\rachel{Need to consistently name and refer to the catalog in some way that more clearly indicates its origin, as noted in earlier sections} \done 

%\rachel{Is that the uncertainty in the shear value, or in $m$ measured using the ensemble shears?}\tianqing{The multiplicative bias},

%\rachel{So is that the number you used?  Precisely 100?}\tianqing{Nah, 100 is the least amount of galaxy pairs in each data-point, it is always more than that.} \rachel{So how many do you use?  I feel I am missing some basics: you have the full catalog.  Then you make a fixed subsample of it - of what size?  And then you cut it up, but always into groups of more than 100, before simulating the 90-degree rotated pairs?  I encourage you to think through the issue of how to make this work reproducible, which means that these topics that are left vague need to be clarified somewhere.}

%\rachel{I suggest restructuring: put this figure with a brief description in Section~3.2.1 when explaining the COSMOS catalog.  Then refer back to it here.  It's not really a result per se, but rather a description of your methodology, so I think it should not go here.}\done

%\rachel{Explain.} \tianqing{Articulate the trend of the parameter here. }



  %\rachel{comment on whether centroids are constrained to the same position for each component} \done

%\rachel{Need to give enough info that this work with S\'ersic profiles is clear and reproducible: need citations and a URL and other identifying information regarding the catalog.}\tianqing{Added citation and URL in the previous paragraph} 

%\rachel{It would be helpful to the reader if you can indicate for which of your simulation sets are the following remarks relevant?}\tianqing{Mention later in this paragraph} 

% \rachel{this would be a convenient place to reference the equation showing the scaling with sample size}\done. 

%\rachel{Cite Massey et al paper (sometime in the 2000s) from the STEP or STEP2 challenge that introduced this concept of shape noise cancellation.}\done 

%\rachel{These last sentences seem like a very long way of saying you are using the 90-degree pair trick, but without really clearly specifying for which simulation sets you do so.  I think this can be substantially shortened but with the key missing info added.}\done

% \rachel{I don't understand what it means that the ensemble would have zero shape biases - we're trying to measure the bias, and it's clearly non-zero}\tianqing{Sorry, I meant to say ``zero average shape'', I have fixed it}. 

%\rachel{No, this is not a limitation - it's the entire purpose of including the 90 degree rotated pair!  There are indeed limitations associated with the fact that you can't measure selection biases effectively, but that's a different issue.}\done. \rachel{Next sentence is off point.  It doesn't affect the conclusions of the study because we have other ways of measuring the errorbars.}\done 
%This, however, does not affect the conclusion of this study, since there are other way to measure the errorbar of the ensemble shear. %\rachel{It would be valuable to explicitly state the limitations of the 90-degree rotation trick, and explain why those limitations don't matter for this study.}\done

%\tianqing{changed the order of narrative in this subsection}

%\rachel{Should clarify that these are the base PSF but not the base {\em effective} PSF.} \done

%\rachel{The description in the next few sentences is not clear.  Do you actually convolve the galaxy with both PSFs, and generate images of both PSFs? Or do you only convolve the galaxy with the true PSF, but make images of both PSFs, so as to measure each galaxy twice?  This text needs to be clarified regarding the actual process.  Think of this as an issue with reproducibility: you would like readers to be able to think there and reproduce your analysis process, so greater precision is needed.}\tianqing{Only convolve with effective true PSF, specified.}

%\rachel{We already defined the `effective PSF', so should the next sentence be simplified?}  

%\rachel{The effective true PSF is perfectly round?  Or the base PSF is round?}\tianqing{The base}\done, 

%\rachel{refer to equation 3?}\done ,
by construction.  %\rachel{Should clarify whether this statement is being made of the intrinsic, round PSF or the effective PSF (after convolving with a pixel response function).} \done \rachel{Hmm, I'm worried about this.  You said that the PSFs have the same second moments, and {\em then} they are convolved wiht the pixel response.  If so, then the second moments of the {\em effective PSFs} consisting of the Kolmogorov/Gaussian convolved with the pixel response are not the same for model and truth.  In other words: it should be the case that you define the effective PSF as Kolmogorov/Gaussian convolved with pixel response, and the effective PSF is what should be forced to have the same second moments.  That's different from what you've written here.  Please can you confirm exactly what you did and, if not what I wrote here, you may need to redo your calculations.  The key point to remember is that the basic Gaussian/Kolmogorov is not what matters, it's that convolved with the pixel response that matters.} \tianqing{Change so that the effective PSFs have the same second moment}

%\rachel{This sentence is only obvious once you say that you define the shear bias by taking the difference between the shear estimation with the {\em model PSF} and {\em true PSF}.  Until you say this, the shear bias could be caused by limitations in the shear inference method.  So I suggest either moving this sentence or clarifying it by adding that information.} \tianqing{I mention the same statement in the previous section, so I will briefly expalain here.}

%\rachel{Throughout the paper: S\'ersic, not Sersic.} \done 

%\rachel{Tianqing: please carefully read and check the next sentence, which I introduced to try to clarify what exactly is being done differently between the true and model PSF.  Is this correct?  If not, can you adjust it to be correct?}\tianqing{Yes, this is 100\% correct.} 

%\rachel{From this brief high-level description, it's hard to understand how you can preserve the 2nd moments when making such changes.  Need to be more quantitative and specific about what you are actually doing, taking it step by step.  Give actual numbers.  Or, refer forward to the section where you will actually explain this - because right now it reads like this is meant to describe what you did (but without enough detail).} \tianqing{Explain steps of resizing below.}

%\rachel{You've not said how you create the modified PSF in this first step.  I {\em think} you simply take the base PSF and introduce the modification of the parameter that you use to control the PSF model kurtosis, without changing the resizing parameter at all.  Is that right?} \tianqing{Correct}

%\rachel{Note that my early comment about locations of hats applies here.}\done 

%\rachel{I think you are introducing too many labels - why not cause these `true' and `model'?  It's true that you will keep modifying this as you iterate to convergence, but still, they are your candidates for true and model PSF.  If you want to distinguish between these candidate ones and the final results, you could use $\hat{\sigma}_\text{base}$ or whatever.  (Note this comment applies until the end of this subsubsection, within and after these bullet points.} \done 
%\rachel{May be worth saying that you do this using a specific GalSim routine, and note that the PSF convolution means that even for a Gaussian base PSF, the $\sigma$ for the effective PSF at this step will differ from that of the base PSF.}\tianqing{I add a short notice here}

%\rachel{I think both of those $\sigma$'s should have hats on them, following on from the step 3 where the hats were used for the effective PSF $\sigma$?}\done, 

%\rachel{Can you confirm the words I've inserted here?  I {\em think} you are modifying the resizing parameter (i.e., S\'ersic $R_h$ or the first Kolmogorov size) but the original text was ambiguous - it sounded like you could be directly applying a dilation to the observed light profile.  Can you fix this to say what you actually did in practice?  i.e. if it's a parameter modification, then remove the equation saying you dilated the profile?  Or if you are actually directly dilating the profile at the image level, remove the words I added, but I suggest being more explicit that `Resize' means `Directly dilate the profile at the image level via interpolation'.} \rachel{Should not use a fraction for an inline equation.} \tianqing{Hmm, I am actually {\em not} using a resizing parameter -- instead, I use the GSObject.resize() function in Galsim. } \rachel{GSObject does not have a resize method in the current method of GalSim. Can you please check this?}\tianqing{Ah sorry, the function is called `expand'. Anyways, I have change the text.}

%\rachel{You have not defined or explained these new symbols $\sigma_{\text{modified}}$  or $\sigma_{\text{base}}$.  There are a lot of $\sigma$ symbols already so I suggest not introducing new ones. Also I think the comparison with the base PSF is a little confusing since you've already defined other symbols for the $\sigma$ of the true effective PSF and model. Perhaps you could avoid defining new symbols by using something  like `until the measured $\hat{\sigma}_\text{model}$ is within $10^{-6}$ arcsec of $\hat{\sigma}_\text{true}$'?} \tianqing{Sorry, this is completely my fault. They are really the same thing, so I just unify the notation.}

%\tianqing{I add this subsection to explain how we approach the problem generally. }

%\rachel{Observers are used to FWHM, so you should quote those rather than $\sigma$ even in cases where you told GalSim a $\sigma$ value.  (This is a general comment, not just here.)}\done \rachel{Not quite what I had in mind.  The point is that a FWHM is not the same as $\sigma$ so you shouldn't call it $\sigma$ - just say ``the FWHM is X\arcsec''.  Also, I really do think this should be done throughout the paper, not just here (I see a lot of places that quote $\sigma$ values).} \tianqing{OK, I change all the $\sigma$ that refer to number to $\text{FWHM}$.} 

%\rachel{Note that if you want, you can simply use an `enumerate' environment and tell latex to label each item as `Step 1', `Step 2' etc. rather than the default `1.', '2.' etc.  This might look neater than bullet points with `Step 1' and so on.}\done

 %\rachel{This is not sufficiently specific to say how you did it: are you including the pixel response?  Is this a process you calculate analytically or is it an iterative and empirical process?} \tianqing{Add some specification}

%\rachel{Here's where I stopped commenting on August 16.}

%\rachel{Need to give basic survey and data release reference; the paper you cited is not about star catalogs - see data release page for list of refs}\done 
%\rachel{This choice of references implies that Bosch et al is a data release paper.  My recommendation is that you preface this sentence with a sentence saying that the dataset we use is from the HSC survey - and cite a few key papers, like the survey definition paper, Bosch+ etc.  Then in this sentence you can just cite the PDR1 paper when referring to PDR1.}\done
%\rachel{say what method is used, and give citations - even if you referred to it in some earlier section, here's your chance to summarize the key features of HSC}\done.

%\rachel{Did you really use only PSF stars - i.e., those that were used to estimate the PSF in HSC?  The text below does not suggest you applied a flag to do so, and indeed you should not do so.  It's important to use all stars that meet your selection criteria so the results won't be quite as affected by over-fitting.  If you did not use a flag to get only the HSC PSF stars, then you should simply call these your `selected stars' (and mention, in 3.4.1, that it includes stars meeting your criteria regardless of whether they were used for PSF estimation)}\tianqing{No, I didn't use a flag for PSF stars in HSC, rather, I have a flag for ``non-extended" object},

%\rachel{One important point that you've omitted is that in HSC the PSF model is estimated separately in each exposure and then coadded using the correct weights to get a coadded PSF.  I think you are comparing the coadded PSF models and coadded images of stars, right?}\tianqing{Right, I add a specification and ref it to the pipeline paper}

%\rachel{Something has gone wrong here - the paper was published in 2018, not 2017, so I think you somehow got an incorrect bibtex reference} \done, 

 %\rachel{If you mean specifically the ones labeled ``Basic quantities and flags' in that table, I recommend saying so explicitly}\tianqing{In the table it says ``Basic flag cuts", and sorry I didn't use all of them so I change this. }. 
%\rachel{I can't tell what the next sentence is saying.  Can you clarify?}\tianqing{We eliminate objects that are poorly exposed with these flags.} \rachel{I am not familiar with the usage of the phrase `poorly exposed' in the astronomical context, only in photography.  I've edited accordingly.} 

 %\tianqing{Can I say the last sentence?} \rachel{It seems like a pretty non-quantitative statement.  I recommend looking at the plot showing the performance of classification\_extendedness in the Bosch et al paper at selecting a pure star sample at the magnitudes that you are working at, and use that to say something a little more precise.}\done %\rachel{surely you must also have an extendedness cut or some other way to get stars?}\tianqing{Yes}

%\rachel{You haven't motivated by 0.1\% was the target.} \done 
%\rachel{I don't quite understand the next sentence; can you please expand/elaborate?} \tianqing{Essentially it is saying, if we are too greedy in measuring highly accurate kurtosis value, we will have too few samples to cover the whole area, and vice versa. }

% Next part is not really necessary.
%The second benefit of setting a lower limit for SNR is that it excludes faint galaxies that are falsely categorized as un-extended objects, which dominate at SNR  $\sim 5$ to $\sim 50$. (a reference for this) %\rachel{also note that a tilde in text mode does not show up; it's a latex special character.  Need to use math mode.} \done

%\rachel{just `star' here and below?}\tianqing{Yes} 

% \rachel{In writing, I don't normally see it referred to this way.  Usually it's more like k-d tree, I think.  Can you please check and if needed, correct this?}\tianqing{I did a little research and found academic papers using all ``KDTree", ``k-d tree" and ``kd-tree". There is paper referring other's ``k-d tree" while calling it ``KD-tree" themselves. So I guess this thing doesn't have a well-unified name. Let's stick with k-d tree since wikipedia use it and most physics people who search it up will see the wikipedia page for explaination.}. %\rachel{with what criteria for determining that it's a double star?  and how were those criteria determined} \done. 

%\rachel{This next sentence suggests you did {\em not} use the entire catalog, only your star catalog, for this cross-matching.  Can you clarify?} \tianqing{I guess I didn't say this clearly: So we search through the {\em entire} catalog, and find all the objects with near neighbors. This forms a ``black list" of stars that we don't want. We then stars in our catalog that are on the ``black list".} 

%\rachel{really only extended? Not stars?  I thought it's from any other object}\tianqing{Right.} 

%\rachel{The horizontal axis should just be `Blendedness' or \code{iblendedness\_abs\_flux}.  The legend should use math mode so you can write $e_1, e_2, \sigma$.  I think the legend is incorrect - $\sigma$ is the fractional residual, not the percent, right?  (`Percent' implies you've multiplied the fractional residual by 100.) The title should say `Residual' rather than `Error'.   Finally, the font in all text on the plot is too small (should be same size as the font in the paper) - try to get it more like figures 2--5. }\done
    %\rachel{I think you need a y-axis label?}\tianqing{Add a label.}

%\rachel{say how this was determined/validated} \tianqing{I may need to do some testing on this criteria.}\tianqing{Honestly, maybe I should apply a blendedness cut much more aggressively: This $10^{-0.375}$ cut is just to veto the galaxy that has unphysically skewed $R_2$ (for galaxy resolution purpose?). For our purpose, the blendedness can be seen as a type of noise and should be kept on the same level as other noises. Should cut at 0.001?} \rachel{The HSC papers that introduce this criterion describe what it's doing.} \tianqing{Change the cut at 0.001, which remove ~7\% of the data} \rachel{OK, but you need to show how you determined this - actually show your plot that drove you to make this cut.} \tianqing{I show the plot the in the results section: Is it ok to refer to later sections?} \rachel{It is, but why not move the plot here?  After all, it's not one of your main science results, but rather a way of justifying the methodology that you've defined in this section.\done}

%\rachel{should this be `typical' i.e. not the best but not the worst?} \tianqing{I think it is the best seeing except the two fields that don't pass?} 

%However, \cite{2018PASJ...70S..25M} shows that the two best seeing field (partly) does not fulfill the requirement of PSF model. 

%\rachel{If the better-seeing ones are better samples for testing the PSF model, why wouldn't we use them?  I don't understand this sentence.} 

%\rachel{Broken reference}\done 

%\rachel{no need to define a symbol $n_s$ for this, as it's never used again}\done, 

%There are  \rachel{You can't use a tilde in the text in latex; it's a reserved character that forces a single space.  Use the `sim' command in math mode.}\done $\sim 2.7$ million objects that pass the flags. Of these, \rachel{Another tilde here.  And MNRAS convention is to use all words or all numbers, so either 80,000 or eighty thousand or $8\times 10^4$.  Same comment applies in the rest of this paragraph.}\done $\sim$ 80,000 object with SNR $> 1,000$.   The blendedness cut further reduces the catalog to 70,000, and there are $\sim$ 2,000 objects that have close neighbors, and therefore eliminated. Overall, we select 68,000 objects for investigating the PSF model. \rachel{Remind what is the area and therefore the number density.  This is important as it gives a sense of on what scales you can reasonably expect to measure correlation functions.} \rachel{Have you considered just making this a table?  i.e. one row is number of stars passing flag cuts, the next is the number passing flag cuts plus SNR cuts, etc.  It seems more useful than a paragraph.}

%\rachel{This section needs a punch line: how many stars passed your flag and SNR cuts, how many stars are in your final catalog after the additional cuts, what is their number density and typical separation (which determines the scales on which the correlation function of higher moment residuals can be determined).}\done

%\rachel{I suggest modifying this title from something very general to something more specific, like `Analysis of HSC star images'}\done


%\rachel{Here too I suggest care in use of the term `PSF star' (see discussion above).  It should probably just be `star'.}\done

%\rachel{This would be a good place for a reminder that these are coadded images and there were corrections for detector effects applied at the single exposure level.}\tianqing{Mention the coadd image and PSF coaddition}

%\rachel{People in cosmology often use `map' to mean something specific: they've used something like healpix or whatever to define the value of something on an equal-area grid on the sky.  Did you actually do that?  Or do you, rather, have a catalog of star positions with true and model PSF measurements?  Should use more specific language even if, informally, we might call either one a map.} \done \rachel{Not sure about this - let's talk} \tianqing{Add more detail here} \rachel{Sorry - I still don't get it.  In this paragraph you talk about measurements for individual stars, and say nothing about a map.  In the next paragraph you talk about a map.  So I still don't see whether you are actually generating a map, or just using measurements for individual stars as a function of their position.}\done \rachel{OK, I see you've fixed it here, but you may want to watch out for it elsewhere in the paper.}\tianqing{Change to avoid using the term map.}

%\rachel{This would be a valuable place to describe the sanity checks you did on this catalog: e.g., comparing your second moments of the stars and PSF models to those provided in PDR1, comparing distributions of second moment residuals to those in the HSC shape catalog paper.  All of this is important to confirm the validity of your selection and measurement process.}\tianqing{Add a sanity check above, should I show a plot?} \rachel{This sanity check is not what I had in mind.  I was proposing that you should show you are capable of reproducing existing results in the literature, which is something you should always do where possible to test your code.  This means comparing with some of the plots and seeing whether you can match the plots regarding PSF modeling quality in the shape catalog paper, rather than doing your own independent test of whether the PSF models meet requirements.}\done

%\rachel{The next two paragraphs are somewhat confusing and need some rationalization of notation.  You first refer to the `residual PSF kurtosis' as the fractional quantity defined in equation 8 -- but then in the next sentence you refer to `residual PSF kurtosis' (same words) and define a new quantity $\delta\rakurto$.  The next paragraph goes even further a defines a very similar looking quantity (but not quite, since it has square brackets: $\delta[\rakurto]$) for something that is mathematically and physically different, the fluctuation of the PSF kurtosis.  Likewise you have $\delta(\sigma)$ and $\delta[\sigma]$ which look very similar but mean very different things. I think this needs some fixes to make notation consistent and clear -- for example, make sure that differences compared to the mean are denoted in a very different way from model vs truth.}\tianqing{Unify the notation} 

%\rachel{Is there a reason not to articulate this in terms of the already-defined quantity $\sigma$?  It seems unnecessary and perhaps confusing to introduce more quantities.}\tianqing{You are right, I shall look at the $\sigma$}. 

%, \rachel{It seems to me that you use this beyond the kurtosis residual (figure 10).  I suggest articulating all of this as something you do for multiple quantities, and use a dummy variable (e.g., $y$, after which you can explain that $y$ is one of the following quantities: \dots).}\done

%\rachel{It is not clear to me why you have defined a new variable $r$ for the kurtosis residual?}\tianqing{My bad, this is from some old text.} 

%\rachel{If you generalize the discussion above then you might not need this next sentence:}\tianqing{I mention this earlier, so I removed it.} 

%\rachel{Since you were just talking about a different set of two-point correlation functions, I suggest making this subsection title more conceptual than technical, i.e., `Bias in weak lensing' or `Bias in cosmic shear'.  (There's nothing incorrect about the reference to two-point correlations, but in this case it's a technical detail that makes the subsection title a little too vague in the broader context of the section.)}\tianqing{title is changed}

%\rachel{In this section you use $\gamma$, but I thought earlier you said you were going to use $g$?  Should be consistent.}\done

%\rachel{The text dives into this derivation without saying what is going on or why.  Need to provide a statement about what you're trying to derive before you derive it.}\tianqing{Start a different subsection since this has nothing to do with redshift-dependent bias. }

%\rachel{I recommend working some of this mathematical justification into the text of this section.}

%\tianqing{Please check if the following sentences are correct.}

%\rachel{Section needs a punch line: now that it's in the methodology section you should explicitly say what are the implications for how you carry out the analysis.}\done


%\rachel{I encourage you to consider whether this is really a result of the paper?  Isn't it simply a justification of one aspect of our methodology, so maybe it should go in the methods section?} \tianqing{It is in the Method section now, and I have change the outlines of both sections}

%The next step of this experiment is to assign kurtosis bias for each galaxies in the CosmoDC2 shear catalog. To better resemble the realistic scenario, the kurtosis bias of the galaxies needs to be statistically identical to that measured by HSC star catalog in Section \ref{sec:realPSF}. Specifically, we generate kurtosis map that has similar 2-pt statistics to the HSC map, by \textit{healpix}. We first measure the auto-correlation function of zero-mean kurtosis bias map of HSC star catalog, fit it by a power law, and perform Hankel transform to get the corresponding angular power spectrum. Secondly, we put the angular power spectrum into \textbf{healpix} and generate a whole-sky map of kurtosis bias, then shift the mean so that it has the same mean as the star catalog. We then assign kurtosis bias to each of the galaxy in the CosmoDC2 catalog by their position in the map. In the upper panel of Figure \ref{fig:cl_gen}, we show the angular power spectrum of the input for the map generation and that of the generated map. In the bottom panel, we plot the generated map for the CosmoDC2 area. 

%With the kurtosis bias assigned to each galaxy and the shear-kurtosis bias slope determined by the redshift, we can calculate the shear multiplicative bias. 

%Futhermore, we can calculate the biased cosmic shear by $g_{obs} = (1+m) g$. We then calculate the 2-pt correlation function $\xi_{+/-}$ of the cosmic shear with both datasets. We divide the entire catalog into three tomographic bins. Bin 1 has redshift $0<z_1<0.5$; Bin 2 has redshift $0.5<z_2<1.5$ and Bin 3 has redshift $1.5<z_3<2.5$. We find out for each tomographic bins, the biased correlation function has an uniform relative bias $\frac{\xi_{obs} - \xi}{\xi}$ across all angular scale. However, bin 1 has a relative bias around $0.4\%$ and bin 3 has a relative bias around $1.0\%$. This leads to around $0.6\%$ redshift dependent bias for the correlation function, or around $0.3\%$ redshift dependent bias for the cosmic shear. According to the LSSTDESC Science Requirement Whitebook, the redshift dependent bias caused by PSF modeling error should not exceed 1\% for Y1, and should not exceed 0.1\% for Y10. We have find out that the shear bias caused by higher order moments of PSF model will exceed the Y10 limit for LSST.  

%\rachel{Since the results section has numerous subsections, it's important to give a brief introductory paragraph with a road map to what is going to happen throughout the section.} \done

%Some of the setup is laid out in Table \ref{tab:specification}. 
%\rachel{This is not a particularly useful reference; there is a lot of stuff in there.  You should label the rows and then for each different result you show, refer to the row in the table that describes the setup for that result.}\done

%\rachel{You slip at times (like here) into past tense.  Should fix to consistently use present tense.}\done

%\rachel{I recommend explicitly using your $\delta\hat{e}$ (or $e$?) notation as a reminder that this is the difference between two quantities.}\done 

%\rachel{Refer back to the table with radial kurtosis values?}\done.  
%\rachel{Here is where you should say how the model PSF was defined - presumably using the S\'{e}rsic trick, but just a single value of kurtosis, in contrast with the next paragraph?} 

%\rachel{Need to specify re: PSF shape.} \done  
%\rachel{Earlier in the paragraph you referred to kurtosis bias, but a Gaussian PSF has no kurtosis.  Need to explain the experiment with more clarity.} \done  \rachel{Sorry, I still don't see it - let's talk.}\tianqing{Add a table in 3.1 and add definition of kurtosis bias here. } 

%\rachel{It seems to me that you can only have learned this if you actually simulated multiple values of $e$.  A single value of $e$ as described in this paragraph does not permit you to distinguish between multiplicative and additive biases. So perhaps you should reframe this: `We used a few fixed values of galaxy ellipticity from X to Y, and found that the shape bias is proportional to the galaxy shape, which means that the shape error caused by kurtosis is a multiplicative bias as expected' (to replace the last two sentences of the paragraph)}\tianqing{Right, I add a bit more explanation, please check. } %\rachel{This is vague and ambiguous: what does `almost proportional' mean?} \done

%\rachel{with a single value of shape?}\done 

%\rachel{refer back to the subsection where you say the steps for doing this}\done.

%\rachel{Am I right that the only difference between this paragraph and the previous one is that you are now varying the level of PSF model kurtosis?  If so, you should say explicitly that this is the only difference between the experiments.}\tianqing{Yes, I state the difference} 

%\rachel{Need to connect the dots a bit more: say those ratios are indicated as G/P in the legend.  Should put some indication of bias=0, for example with a dashed horizontal line.  Vertical axis ratio appears to be incorrect: `lensing shear' should be `shape'} \done
    %\rachel{These wordy axis labels are good for talks, but for a journal article, you should use symbols (and expand into words in the caption).  So, this should be $\delta \hat{e}/e$ and $\delta\rho^{(4)}/\rho^{(4)}$ or $B[\rho^{(4)}]$.  Also, I suggest using the actual values rather than the percent.  Finally, the legend should be something like $\sigma_\text{G}/\sigma_\text{P}$ so it's very clear that these are the size ratios of Gaussians.}\done

%\rachel{re-Gaussianization?}\tianqing{Yes}.

%\rachel{Let me reiterate my suggestion that you try a log axis for $\sigma_G/\sigma_P$. Whenever you have a function that changes strongly for small values and not much for large values, a log axis can be a more useful way to visualize it.  I would do that for any of the plots that has some measure of size as the horizontal axis.}\done
%\rachel{There are some opportunities to use consistent notation, which will avoid confusing your readers.  First, you have G/P in the previous plot, and $\sigma_\text{galaxy}/\sigma_\text{PSF}$ here.  Are these the same quantity?  If so, I suggest using consistent notation for them.  If possible, it would be useful to clearly indicate whether this is the measured size based on second moments, or the input $\sigma$ (was not clear to me given that Kolmogorov profiles do not have an option to input $\sigma$).  Second, in the previous plot solid lines and dotted lines were used for re-Gaussianization and metacalibration, but here you've changed the line styles -- why not use consistent ones as the previous plot?} \rachel{The vertical axis has `m' in it, but people typically use that for an ensemble shear bias, and I think this plot is for galaxy shapes?  If so, I suggest using $\delta\hat{e}/e$.}\tianqing{I have change the notation for consistency. Change the $m$ to $\delta e / e$, and change the line style in-line with the previous plot.}
%\rachel{Linear, regauss, and KSB are all moments-based methods, so the fact that they agree in shape pretty well is not that interesting.  I recommend reducing clutter by just showing the two regauss and two metacal curves, since those methods have truly different assumptions.  The plot will then be easier to read.  In the text, you can assert without showing that these other moments-based methods behave similarly, and reduce the amount of discussion on those methods.} \rachel{Still seems to have all the curves?}\done 

%\rachel{General comment on the figure: the plots have the same title, legend, x- and y-axis labels.  It therefore appears that the exact same thing is being plotted.  Reading the caption, it seems to me that the left is galaxy shape bias and the right is weak lensing shear bias.  If so, I suggest indicating this clearly in the y-axis label -- use something like $\delta\hat{e}/e$ rather than $m$ in the left panel.}\tianqing{I have unify the x-range, x-label, y-range and left only one legend. I change the title to what the subject is.}  \rachel{This looks nearly perfect, except there are still two legends with different terminology.  I suggest keeping the left legend and not the right one.}\done 

%\rachel{There are no dashed lines on this plot.}\done

%\rachel{Plot title says it's a Gaussian}\done.

%\rachel{Turn horizontal axis into log for consistency with fig 4?}\done
    %\rachel{You only need to put the legend on one panel, not both.  I suggest that within the legend you call it `S\'{e}rsic n' rather than `sersic index'.}\done
    %\rachel{When you have two side-by-side plots, it's useful to either unify the y axis ranges, or explicitly remind the reader in the caption that the y axes differ.  Is there a good reason why the x axis ranges differ as well?  It seems to complicate comparison for no reason that I can see.}\done \rachel{I see the y axis ranges were unified, but the x ranges still differ. }\done
    %\rachel{consider showing only Gaussian or only Kolmogorov to reduce clutter, and then comment on the one you don't show as additional info in the main text.}\done \rachel{I suggest doing the same thing on the left panel as well, and eliminate the legend on one panel since it's the same color scheme for both.  Or if you want to keep the legend on both, make it consistent.} \done

%\rachel{Why variance?  Why not total range or standard deviation?  Variance doesn't have the right units to plot meaningfully here, and I think for this purpose the total range is most meaningful.} 

%\rachel{Turn horizontal axis into log for consistency with fig 4?}\done
    %\rachel{What are you bootstrap resampling?  Are you drawing a new subsample from the COSMOS catalog each time?  Or do you have a fixed subsample that you bootstrap resample?}\tianqing{It is the latter one.}   
    %\rachel{Left panel needs a label indicating that it's the same population as in the right panel but without any division by S\'{e}rsic index.  Also, I recommend against using the same color for the points in the left panel and one of the subsamples in the right panel - it implies they are the same, when they aren't.  Finally, the x-axis labels on the left and right panels differ.  Are they really binned based on a different quantity, or should it be fixed so they are the same?} \tianqing{Change the color of the left hand to black (And all other plots that use all population.)}
    %\rachel{Vertical axis range doesn't include all points.  Adjust it?} %\rachel{Horizontal axes refer to `half light radius' and `galaxy size', implying these are different quantities.  Should unify (if the same quantity was used) or clarify what measure of galaxy size was used.  I don't think the same quantity can have been used, though, since the left plot suggests the overall population goes through the point (0.2, -3) and the right plot has no sample going through those points - so this seems confusing.} %\rachel{Since the figures are right next to each other, I also recommend seeing how it looks if you force them to have the same vertical and horizontal axis ranges and aspect ratios and font sizes, making them more easily comparable. Perhaps omit the title on the right plot?} \rachel{Should have a single sentence takeaway of the key conclusion from this plot.}\tianqing{I used the flux radius, but it's after HST's PSF: So it wouldn't change the size too much. }
%\rachel{Should say what errorbars represent; the answer differs for horizontal versus vertical errors, I think.}\tianqing{Yes, the horizontal is variance and the vertical is bootstrapping error on the mean value. }


%% Paragraph below is redundant -- just folded one phrase into the paragraph above.
%From Figure~\ref{fig:GGlinear}, we can tell that the relations between multiplicative error and kurtosis bias are linear, and the slope of the line depends on the size ratio between the galaxy and the PSF.    %\rachel{More than that: it's not even monotonic, which is worth noting explicitly.} \done 

%\rachel{The text after this doesn't seem really related to the figure: it's not clear how the two pixel sizes mentioned here are indicated, and there definitely are not five different shape measurements.  I've not edited the next few sentences in any detail, but I suggest rewriting to more clearly describe this figure.} \tianqing{I fix it.} 

%\rachel{You should comment on any challenges in comparing these results.} \done

%\rachel{In what follows, it is not clear to me why the paragraph now switches back to talking about figure 2; is this meant to talk about figures 2 and 3 together?  I've left the text as-is but suggest you clarify or move it (if it's really only about figure 2).}\tianqing{Ah sorry, I think I use the wrong figure label, it is meant to talk about Figure \ref{fig:GGsize_ratio}.} 

%We show the results of the re-Gaussianization in solid and Metacalibration in dash-line.

%\rachel{It sounds like you're saying `we use A and B as the default', which doesn't totally make sense to me.  Can you clarify?}\tianqing{You are right, they are not always used. I change the description.}

%\rachel{Actually, I find this plot rather concerning; the Kolmogorov result does not seem to be converging to 0 bias at large size (it seems to be flattening at a non-zero value even for galaxies that are 10x the size of the PSF).  Can you please check whether this is true?  If so, I think there must be a bug.} \tianqing{I check for $\sigma_{G}/\sigma_{P}$ over 20, it seems that it just converge to 0 really slowly.} \rachel{OK, so you should comment on this in the text.  Otherwise it's a pretty obvious question for any reader that is left unanswered.}\done

%\rachel{For the sake of precision, you may wish to say it's a galaxy model with one more free parameter rather than saying it is `slightly more complicated.'}\done 

%\rachel{This paragraph says it is about figure 4, but it seems like it is really only about the left panel.  Is that correct?  If so, I suggest saying that explicitly.}\done 

%\rachel{You use other notation on figures, for example `HLR'.  Should homogenize notation across text and figures.}\done 

%\rachel{It is worth noting that the index=0.5 case is the same as was presented in Fig.~\ref{fig:GGsize_ratio}, I think.}
%\rachel{Some of the curves appear to be steadily increasing as the galaxy-to-PSF size ratio increases, which seems worrisome.  Can you check that they do at some point go to zero?} 


%\subsection{Galaxy Rotation pair}
%\rachel{This subsection title is describing the technical detail of what you did, but it's missing the substance: correct me if I'm wrong, but I think that the point here is to talk about the impact of HME on ensemble shear estimation.  Perhaps the title should reflect that, rather than the technical details of how you carried out this test?  Or, alternatively, what would you say to absorbing this very short section into the previous one, changing the title of that to indicate you will cover shape and shear biases, and modifying the narrative to show the progression from one topic to the next?} \tianqing{I think it makes sense to combine 4.1 and 4.2.  So I just change the title of 4.1 to ``Impact on single galaxy shape bias". We can interprete the galaxy pair of a technique to cancel out the shape noise. } \rachel{Fine to combine them, as I said, but the title is then wrong.  You don't explore only single galaxy shape bias; you also explore shear inference bias.}\tianqing{Make the title ``Single Galaxy Experiments''}

%\rachel{$e_1$?} \tianqing{Yes} 

%In order to eliminate shape error in this special scenario, we create a 90-deg rotation pair for the galaxy and apply the same shear. 
%% Note: you already explained your methodology, so you don't need to explain it in much depth again.

% \rachel{Plot title says it's a Gaussian PSF} \done. \rachel{I don't think this is possible, since the left is shape bias and the right is shear bias, right?} %\rachel{broken ref} \done 

%And the shear of the 90-degree rotated pair is measured as described in Section~\ref{sec:shapemeasurement}.
%\rachel{One important issue with this is that in section 3.3, you never said how to measure the ensemble lensing shear for re-Gaussianization - you only did for metacalibration (which has a different shear estimator).  So I think for this plot you should either show metacalibration, or you should update section 3.3 to include text on shear estimation with re-Gaussanization.}\tianqing{I add some text in Section 3.3 to say about shear of 90-degree pair and ensemble shear.} \rachel{OK, let's leave this note for now, I will go take a look later.} 

%\rachel{But if you're going to use ensemble shear for the rest of the paper, you should mention that.}\done   %\rachel{Since you have absorbed this into section 4.1, should just say `from earlier in this section'.}  \done %\rachel{Consider putting figures 3 and 4 as two panels in the same plot right next to each other to make the comparison even more straightforward.  You could also then avoid having a legend on both, if you use consistent color schemes.} \done

%\rachel{Note: I edited/commented up to here.}

%\rachel{Similar to my comment on the previous subsection, I suggest changing the title of this subsection to reflect what new information you were trying to obtain, rather than the technical details of how you tried to obtain it - so, something like `Impact of HME on realistic galaxy populations'?} \done

%\rachel{It's not clear to me what the quotation marks are doing in the subsection title.  Are they necessary?  I'm also not sure that the word choice is particularly descriptive - so, let me reiterate my previous suggestion that you call it something like `Experiments with realistic galaxy ensembles' to contrast it with your single-galaxy experiments.  Finding concise but descriptive subsection titles is valuable in helping people navigate your paper, but it does take some thinking.}\tianqing{Change to Experiments with realistic galaxies.}

%\rachel{Equation reference is broken, because you tried to refer to something defined using equation* (which by definition will have no number).  Need to convert it to equation, so you can refer to it.  With that said, I would recommend indicating the cut in the section where the catalog is defined, rather than here.  It's part of your methodology for how to use the catalog.}\tianqing{I move the sentence to the method section}


%\rachel{Sorry if I missed it, but I do not think you have said what cuts you used on the simulated galaxy sample?}\tianqing{Just one cut on resolution factor, I state it in the method section. }

%\rachel{I don't quite understand the numbers in the next sentence (what is the 0.01?).  Can you clarify?} \tianqing{Ah, my bad. It means we only test for $g_1<0.01$, and $B[\rakurto]$, I change the sentence.} 

%\rachel{missing end of sentence?}\done

%\tianqing{I move the method of determining error bar to the method section. }

%\rachel{You need to explain what you did to make this figure: i.e., that instead of drawing random subsamples of the catalog, you drew galaxies within ranges of galaxy size and S\'{e}rsic index, and measured ensemble shear biases using these subsamples.  What PSF did you use? Also, you should say whether this is metacalibration or re-Gaussianization. (I encourage you to think carefully about how much of this info to have in the text and caption, versus just the text.)}\tianqing{Sorry I didn't put everything here, but: the ways that we draw sample from the ensemble is at Section~\ref{sec:galaxyprofile}, same as the way we get the errorbars. PSF, shear, shear measurement method and kurtosis bias are the common feature of these results, so I say them in previous paragraphs.} 

%\rachel{It's noticable that previously you said it was the galaxy-to-PSF size ratio, but here you just say galaxy size.  Was this simulation done with just a single target PSF size and pixel scale?  Should we be reading this as the same conclusion, or a different one from before?}\tianqing{I clarify that this agree with our previous conclusion} 

%\rachel{I recommend articulating this in terms of the Sersic index being an important secondary factor.}\done \rachel{I think this narrative in the previous paragraph now changes with the updated plots?}\done

%\rachel{The next part should be rewritten.  Please re-read the relevant parts of the appendix of the doc that is cited - your description of the impact of redshift-dependent shear bias is incorrect.  There is also another paper you should cite (you can find a reference to it in the doc you are citing).  This is an important conceptual point, not a minor correction, so I am asking you to do it (learning experience), unlike many of the language edits I've been making directly.}\done 

%In Fig.~\ref{fig:great3_bin_property}, we show a polynomial fit for $m/B[\rho^{(4)}]$ as a function of redshift. The order of the polynomial fit was chosen based on the Akaike Information Criterion (AIC) \rachel{with what threshold?}, which motivated selection of a fourth order polynomial. The best-fitting function is $m(z)/B[\rakurto] = -1.10 + 0.92z - 1.80z^2 +0.55z^3 -0.05z^4$. In Section~\ref{sec:redshift_dependent_bias}, we will further discuss the consequence of such redshift-dependent multiplicative bias, combined with the results shown in Section~\ref{sec:realPSF}

%The main parameter that affects the shear bias binned by %F814W magnitude (right panel of Fig.~\ref{fig:derived_quant}) is also the size of the galaxy: brighter galaxies tend to be larger in apparent size. As a result, fainter galaxy bins have a more negative ratio of shear bias to PSF kurtosis bias. % \rachel{In case it's not clear to a reader why you say size and sersic index are primary/secondary determining factors of the bias, you might want to point out that the shear bias varies with them more strongly than with redshift or apparent magnitude.  Also, should briefly explain the trends in terms of figure 5.} \rachel{You can make a stronger statement than this about cosmological parameter biases - point at previous papers that showed that redshift-dependent shear calibration bias causes a bias in cosmological parameter determination.} \tianqing{Explained the trend, and briefly layout the results and importance of redshift dependent bias here. Since we have a different section on this, I didn't write very much about it here. }
%\rachel{Do we use or rely on this conclusion much?  If not, I think we might want to omit the right panel of that figure and simplify the text accordingly.}\tianqing{There is no conclusion based on this result, so I will remove it.}

%\rachel{The next sentence needs some updates; see my comments on and updates to a similar sentence in the caption of Fig.~\ref{fig:great3_bin_property}.} \done 

% \rachel{I suggest unifying the vertical axes since these are side-by-side panels.}\tianqing{No longer have two panels} %\rachel{Say what band, and make sure label and the figure text in general is clear these are photometric redshifts, not true redshifts.}\done

%\rachel{Font size for axis and tick labels looks smaller than paper font size.  Should check/fix this.}\done
    %\rachel{This quantity $B$ was defined in an equation, and it was {\em not} a percent.  I think it is confusing to change how it's defined in a figure compared to the equation, so I suggest modifying the color bar labels to indicate the values of $B$, and the caption to refer to the fractional residual rather than a percent (and give a direct reference to the equation defining $B$).}\tianqing{I change the colorbar and called the B ``fractional error''} 
    %\rachel{Since the top two panels are plotting quantities that should be consistent, I suggest using identical colormaps and color bars for the top two panels.}\done 
    %\rachel{Can you clarify whether this plot was made by literally plotting a point for each star, or are you averaging within healpixels of some fixed size?}\tianqing{It is plotting one point at each star.}

%In this section, we show the results for the PSF higher moments modeling quality for the HSC shear catalog described in Section~\ref{sec:hscdata}. We pick out the bright stars to evaluate the light profile of the true PSF, we then look at the PSF model generated by the PSFEx as the model PSF. The relative difference in the model and the truth is referred as residual, or kurtosis bias.   %\rachel{Refer back to whatever section defined your selection criteria and other aspects of the methodology that led to the results in this section} \done

%\rachel{Do you only use this field for all of your results?  Or do you use the full catalog for most plots, and just use this field for the maps?} \tianqing{I only use this field.} 

% \rachel{Seems smaller than that - maybe 2.12-2.22, which is 0.1/2 or about 5\%?}\tianqing{Yes}, 

%\rachel{This would be a good place to refer to table 1 in interpreting these numbers} 

%\tianqing{Use preciser term here.}  %\rachel{Need a high-level takeaway: what's interesting / why are you showing this?  You seem to have it later on (`From the kurtosis map\dots' but it's really worth having it here.  You can use it to motivate a statement that we have to then quantify the one- and two-point statistics of these quantities.} \done 

%\rachel{I encourage you to consider some restructuring: since you've already said that for weak lensing shear biases we only care about the average kurtosis bias (back in section 3), you could remind the reader of that point, and simply quote the average kurtosis bias, putting the rest of these plots and discussions into an appendix.  The reason I think this is worth considering is that the rest of this section doesn't ultimately contribute to the narrative flow of the paper; it's a detour to understand a finding, but it doesn't change how you use that finding.  Appendices are a good place for that kind of thing.}\tianqing{I have put the discussion of one- and two-point statistics into appendix.}

%\rachel{I think at some point in this subsection or elsewhere, you need a clear caveat on your methodology: while you showed the simulation results are not {\em too} different for different base PSFs (Gaussian, Kolmogorov), it is the case that the HSC PSFs are not precisely like either of those base PSF models.  Hence the connection between the simulations and the HSC analysis is approximate, and the results here should be considered as having some uncertainty at the tens of percent level.}\tianqing{I add a paragraph after Eq~\ref{eq:m0}}

%\rachel{You need to motivate your new approach using just the average kurtosis bias.  I think the motivation, mathematically, goes something like this:}
%\rachel{You don't need Fig.~\ref{fig:slope-redshift} at all; you could simply show this fit on Fig.~\ref{fig:derived_quant} and move the description of the fit into the section where Fig.~\ref{fig:derived_quant} is described.  Then you can use the fit here without having to introduce a new figure.  I realize the redshift binning differs for the two figures, but I think that is not enough to justify an entirely new figure.  Instead, I suggest that you choose which binning best tells the story when including the fit, and use that in Fig.~\ref{fig:derived_quant}.  (So I did not edit the caption of Fig.~\ref{fig:slope-redshift}.)}\tianqing{I have remove that Figure, and add a linear fit to the shear-redshift plot.}

%\rachel{Avoid phrase `distance of redshift' since redshifts can be converted to distance (so people might think you mean cosmological distance).} \rachel{Pick one of the curves, and give the formula for it here.}
%

%% This section is very short, so I don't think you need to provide a spoiler.  You can simply walk through the result and explanation.
%We show that after dividing the above requirements by 3, the biases caused by errors in higher moments of the PSF (with current PSF modeling methodology in HSC) satisfy the Y1 goal, but pose a challenge for LSST Y10 requirements, motivating further improvements in PSF modeling methodology.  

%\rachel{The essential background to this whole paragraph is that you're using the mean kurtosis bias in HSC and ignoring spatial fluctuations. This is a good place to work in the justification based on the explanation I put at the top of the section.}

%\rachel{should explicitly reference figure on this from previous sections, to remind where this comes from}.




%\rachel{Note: I turned a few $\mathbf{z}$ to $z$ because redshift is not a vector quantity.}\tianqing{Noted}

%To relate this to $m_0$ in Eq.~\eqref{eq:m0}, we assume the highest tomographic bin for LSST will have a central redshift of $z=2$.  The total variation in redshift-dependent shear bias across $z=0$ to $z=2$, after multiplying by the mean kurtosis bias from HSC ($10^{-3}$; Subsec.~\ref{sec:realPSF}), is 0.002.   This corresponds to $m_0=10^{-3}$.  

%\rachel{We should consider reiterating here that PSFEx is not the planned algorithm even for LSST Y1  This is important context.} \tianqing{I said that at the end of this Section.}


%\rachel{Edited up to here!}

%\rachel{The conclusion is a place where you can briefly summarize your results in the broader context.  As such, I would recommend having just a few selected references for that broader context -- e.g., the standard second moments formalism that you're going beyond.  I think more than a single sentence comparison to the Schmitz paper is also warranted (compare your key conclusions against that paper in a paragraph that briefly describes their methodology).  In general, if your results differ, you should have some attempt at explaining why.}\tianqing{Add a bit more explaination to the difference}


%\rachel{Note that in the conclusion, it's acceptable to use past tense since you are summarizing what you already showed (see edits below).}\tianqing{Thanks.}

%\rachel{Should say implications of this result in the broader context of this field.  This includes implications for PSF modeling algorithms, for DESC testing suites (i.e., they should incorporate tests of this effect), for current surveys (your results suggest DES/HSC/KiDS don't need to worry about this), and for your future work (which includes quantifying the impact of higher moments of the PSF more thoroughly).}

%\rachel{This paragraph seems to repeat the previously-described results without adding anything significantly new.  Can it be omitted entirely? (Note: I did not edit it.)}\tianqing{I think so.}
%Generally, we can make several comprehension of the results. First, the HME of PSF model can cause significant bias for weak lensing shear if not modeled well. Secondly, The amount of shear bias caused by HME depends on the distribution of galaxy size, and S\'ersic index. Lastly, the PSF modeling error in the case of first year HSC catalog indicates that the level of the shear bias caused by the HME of PSF is around $0.1 \%$. This place the requirement for higher moment modeling quality for later PSF model algorithms. 

%\rachel{This paragraph also repeats a number of points from before.  I think really only the last two sentences are new, and they could be incorporated into the paragraph I suggested above on broader implications of your work.  (Note: I did not edit this.)} \tianqing{I have written a broader conclusion and integrate this paragraph into that.}
%This paper is also restricted in several ways. First, we are not modifying one single higher moment of the PSF at a time, but rather changing all the radial higher moments and use the kurtosis as the measurement of the amount of error. Secondly, we are only investigating in the HME that causes multiplicative bias. Other HME might cause additive bias, furthermore cause scale-dependent error in the two point statistics. We are aiming to investigate these questions in the future research. 

% ----------------------------------------------------------------------
%\section*{Contributors}

%\rachel{You should not have a separate section for contributors.  Rather, put the contribution statements required by DESC in the acknowledgments, after funding acknowledgments.}\done

%\rachel{Acknowledgments should be a section, not a subsection.}

%\rachel{Here is where you can put contribution statements.  For example, something like this: TZ developed the software, carried out the analysis, and led the writing of this paper.  RM advised on motivation, scope, experimental design, and analysis, and edited the paper draft.}\done

%\rachel{The ordering here seems a bit chaotic. This is a DESC paper that used HSC data for part of the work.  So, I suggest putting the DESC acknowledgments first, then the statement that the work is based in part on HSC data, then the HSC acknowledgment.} \done

%\rachel{You've listed 3 plots but there are four plots.  I wonder if you might want to actually reduce the level of specification - just say that there are 1D and 2D histograms of the PSF kurtosis (true, residual) and its connection to PSF size?}\done. 

% \rachel{Same concern, I don't see how the plot can show you this when it's about PSF size residuals rather than PSF size.} \tianqing{I change the plotted quantities so that it reflect the PSF size.}. \rachel{Overall it seems like this text is not really talking about the key conclusions from the panels that are actually shown in the plot; this paragraph and plot need some work.}\tianqing{I have change the notations, renew the plots and change the texts to be clearer.}

% \rachel{I don't see how the plot shows you this.  You don't show anything about PSF size, just PSF size residuals.}. 

%\rachel{In general?  Or on average?  In other words: is this a statement about something that is generally true in all cases, like a coherent shift of the distribution?  Or is it a statement about mean values?  I think it is the latter?}\tianqing{Yes, ``on average'' is better.}

%\rachel{I suggest putting vertical lines at the median or mean values, so people can read them off more easily.} \done 

%\rachel{I think you should carefully revisit notation for these axes.  First, perhaps some of them could be $B[\rho^{(4)}$, a quantity you already defined.  Second, `Truth' should be 'True'.  Third, perhaps `Kurtosis' should be $\rho^{(4)}$.  There might be other changes worth making.  Is the color scale actually meaningful?  If not, I suggest removing the colorbar and simply saying it's a linear scale in the density (with the maximum value differing per panel).} \rachel{Watch out for cases where your tick labels are overlapping.  In those cases you should force it to label less often.} \rachel{The caption refers to panel locations like `top right', but this is a single-column figure, so those labels need to be fixed.} \tianqing{I have fixed these issues.} %\rachel{axis labels say `residue'; should be `residual'.  Is `kurtosis residual (\%)' in the top panel and `kurtosis model residue' on the bottom panel meant to be the same thing?  If so, should use the same terminology.}\done %\rachel{I recommend making this full page width, and indicating the medians on all panels.}\done

%\rachel{Need to explain the vertical lines.  Also, there are really too many data points to use only 10 jackknife patches.  Need either more patches, or you should make your bins wider in $\theta$ so you have fewer bins.} \tianqing{Is 20 bins enough? I cannot find a reference to find the appropriate number of bins in terms of data points.} \rachel{Chris Hirata has a paper in 2003 or 2004 that talks about this in the context of bootstrap (but the considerations are the same for the jackknife).  Roughly speaking if you have $M$ data points, you should have at least $M^{3/2}$ patches to avoid significant noise in the covarianace, or at least $M$ to avoid the covariance matrix actually being singular.  I would recommend reducing your number of $\theta$ bins to get around this problem. \tianqing{Changed to 10 data points: $10^{1.5} =  31 $}} %\rachel{I recommend making this 1.5 times the column width.  There's too much detail to cram into a single column.} \rachel{Put a vertical dashed line corresponding to the extent of the FOV?}\done


%\rachel{In this paragraph you've deviated from some of your typical notation, e.g., $Bias[\rho^{(4)}]$ instead of $B[\rho^{(4)}]$, and you've called the PSF size $r$ for the first time that I noticed.  I suggest carefully revising this to be consistent with the rest of your notation and with standard practice.} \done

%\rachel{The errorbars look super wrong, but I know you investigated this, so you should explain why they appear so over-estimated.}  \tianqing{A question here: The treecorr gives the variance of the xi, not the error, are they the same, is what we see actually the variance instead of error?} \rachel{Treecorr gives variances, and you should be plotting their square root (standard deviation); they look a lot larger than shot noise errors because large-scale systematics induce coherent fluctuations across the HSC survey area.  So you should explain this.}\done 

%\rachel{What's interesting is that nearly all correlations drop to zero above this scale, but one of the panels shows relatively little decrease - should comment on this explicitly!}\tianqing{Ah, in the new version, all the correlation function drop to zero at $100 \arcmin$, since I am plotting the zero-averaged bias.}  

%\rachel{it implies; generally, people infer something (e.g., `from this plot, we infer that\dots') but data and plots do not infer things}\done 

% \begin{figure}
%     \centering
%     \includegraphics[width=0.98\columnwidth]{plots/unweighted_size_ratio.pdf}
%     \caption{Slope of shear-kurtosis bias for ensemble of galaxy binned by redshift, where blue bins have uniform redshift division between bins and orange bins have equal number of galaxies in all bins. The curves are the polynomial fittings to the $4^\text{th}$ power. The error bar of the horizontal axes shows the variance of each bin, while the error on the vertical axes shows the error on the mean value, generated by bootstrapping for $10^4$ times. }
%     \label{fig:slope-redshift}
% \end{figure}


%\input{desc-tex/ack/standard} 



%\rachel{Some stylistic and content advice:
%\begin{itemize}
%
%    \item \rachel{I changed this a few places in the intro, but more generally, I encourage you to avoid using the term `systematic error'.  You sometimes used it when you meant a systematic bias (i.e., a well-defined offset from the true result) and a systematic uncertainty (i.e., due to mismodeling we can't say for sure whether we should have an unbiased result).  The terms `systematic bias' and `systematic uncertainty' are more precise and will cause less confusion.  I encourage you to look for the other instances of `systematic error' in your paper and fix them.} \tianqing{Fix the obvious ones. I will leave this comment here so I always keep an eye on.}
%
%    \item \rachel{There is some value in using consistent styles in the plots.  For example: you have 2D histograms in figures 6 and 9 that have a very different look - consider using the same style?  And many of your 1D plots use the same color palette, but not figure 11 - can that one be made consistent?}
%
%    \item \rachel{To avoid issues with reviewers and journal editors, I recommend glancing over the MNRAS author guide, \url{https://academic.oup.com/mnras/pages/General_Instructions}, and getting the paper consistent with it after your next round of editing.} \tianqing{I have take a look, will revisit this later.}
%
%        \item For the next stage of iterating on the paper, and before circulating this within the DESC PSF WG, I recommend moving the large commented-out blocks of text and discussion into a separate tex file (or deleting).
%
%\end{itemize}}
%
%\tianqing{
%Some general questions
%\begin{itemize}
%
%    \item Remind myself to put (a) (b) etc. on different parts of the figure. 
%\end{itemize}}


%Measuring the convergence directly would generally require assumptions about the pre-lensing galaxy sizes \response{and/or magnitudes}, whereas measurement of shear relies on the fact that galaxy shapes are generally presumed to be randomly oriented\footnote{This assumption is broken by intrinsic alignments \citep[e.g.,][]{2000ApJ...545..561C, 2000MNRAS.319..649H} -- the correlated galaxy alignments due to local effects such as tidal fields.} in the absence of a coherent weak lensing shear signal. 
% Eq.~\eqref{eq:sheardef} is commonly written as 
% \begin{equation}\label{eq:sheardef2}
% \begin{pmatrix}
% x'\\
% y'
% \end{pmatrix} = (1-\kappa)
% \begin{pmatrix}
% 1-g_1  & -g_2  \\
% -g_2 &1+g_1
% \end{pmatrix}
% \begin{pmatrix}
% x\\
% y
% \end{pmatrix}, 
% \end{equation}
% in terms of the reduced shear $g_i = \gamma_i/(1-\kappa)$ \citep{dodelson_2017}.  

% The expected shape noise uncertainty $\sigma_{\langle \gamma \rangle}$ when measuring shear using $N$ galaxies in some region of the sky is
% \begin{equation}
% \label{eq:shapenoise}
%     \sigma_{\langle \gamma \rangle} \sim  \frac{\sigma_{\gamma}}{\sqrt{N}},
% \end{equation}
% where $\sigma_{\gamma} = 0.28$ \citep{2018arXiv180901669T} is the per-galaxy and per-component intrinsic shear dispersion.   
% Deeper surveys see more galaxies in the same region of sky, decreasing the shape noise. 
%  The cosmic variance can be mitigated by increasing the area of the survey. However, we are not able to completely reduce cosmic variance since we only have one instance of sky to be observed from the Earth. 


% \cite{2010MNRAS.404..350R} and \cite{2016MNRAS.460.2245J} 
% described how spatial correlations in the PSF model shape and size residuals propagate to the weak lensing shear-shear correlation functions used for constraining cosmological parameters. 
% The multiplicative biases of the weak lensing shear correlation functions are independent of angular scale, while the additive biases are described as five correlation functions of the PSF second moments and their residuals, also referred as ``$\rho$-statistics".  
% The biases on weak lensing shear-shear correlation can be estimated and requirements on them placed if the PSF modeling error is well-quantified \citep[e.g.,][]{2016MNRAS.460.2245J, 2018PASJ...70S..25M}. However, systematic uncertainties on the PSF modeling errors lead to shear biases that must be marginalized over \citep[e.g.,][]{2020PASJ...72...16H}. 


%In other words, the formalism would predict zero weak lensing shear systematics as long as the PSF model size and shape match the true PSF size and shape, regardless of how well the  higher moments of the PSF are modeled.
% In \cite{2020A&A...636A..78S}, additional multiplicative and additive biases were found on top of the prediction by the second moments formalism for the space-based telescope \textit{Euclid} \citep{Euclid_overview} 
% when using a realistic PSF model for that telescope.  
% The additional shear biases are likely caused by HME of the PSF modeling. However, there is little discussion on how these additional shear bias depend on the details of the HME 
% of the PSF model.
%There is also little exploration of how the spatial correlation of the HME of the PSF model propagate to the shear-shear two-point correlation functions.


%In Section~\ref{sec:2pt_correlation_bias} we describe our method for combining the results from the simulations and the real data to predict the level of weak lensing shear bias in the two-point correlation functions used to constrain cosmological parameters.  


% Metacalibration works by resimulating the galaxy to be measured with an artificial shear (and a slightly larger PSF), so as to measure the matrix response of the shape estimator $\hat{e}_i$ to the artificial shear $g_j$, $\partial \hat{e}_i / \partial g_j|_{g = 0}$. 
% The response matrix, denoted $R_{ij}$, is calculated as
% \begin{equation}
% R_{ij} = \frac{\hat{e}_i^+ - \hat{e}_i^-}{2 \Delta g_j},
% \end{equation} 
% where $\hat{e}_i^+$ is the measured shape after we add an artificial shear $\Delta g_j$ and $\hat{e}_i^-$ is the shape after we add an artificial shear $-\Delta g_j$.  
% After we calculate the matrix response of the galaxy ensemble, the ensemble shear 
% $\langle g \rangle$ is estimated using the average shape $\langle e \rangle$ and the inverse of the average matrix response $\langle \boldsymbol{R} \rangle ^ {-1}$ via
% \begin{equation}
% \langle \hat{g} \rangle = \langle \boldsymbol{R} \rangle ^ {-1} \langle \hat{e} \rangle . 
% \end{equation}
% \response{The $\hat{e}_i^+$, $\hat{e}_i^-$ and $\hat{e}$ need to be measured by some ``base method''; here we use re-Gaussianization as our base method. }




%Note that the flux radius is the galaxy radius after convolving with the HST PSF, which has an intrinsic radius of $\sim 0.085$\arcsec in the F814W filter \citep{2007ApJS..172..196K}. 
    %\rachel{There is a noticably large amount of white space in this figure.  Might you explore the option of shrinking the gaps between panels and enlarging the panels themselves so that a higher fraction of the figure is taken up by the plots?} \done %


 %\rachel{Not clear to me what it means to compute the average FWHM as a function of seeing?  Do you just mean that you used your measured PSF moments to compute the average seeing in the survey?}\tianqing{Meant to say $f_{\delta \sigma}$} over \code{Healpix} pixels, as a function of seeing, and find similar results to \cite{2018PASJ...70S..25M}. These validation tests of our measured second moment sizes suggest that our star samples reflect the true effective PSF profile.




%We also study the correlations between the following quantities: true PSF kurtosis $\rakurto$, model residual PSF kurtosis $ B[\rakurto]$ and the size of PSF $\sigma_P$. 
%The study of correlations can provide some insight into the circumstances under which the higher moments of the PSF are modeled less effectively.

% We use the two-point correlation function (2PCF) $\xi(\theta)$ to capture the spatial structure of the zero-averaged version of the above-mentioned quantities, including the fluctuation of the true PSF kurtosis $\delta[\rho^{(4)}] = \rho^{(4)} - \bar{\rho}^{(4)}$, the zero-averaged residual kurtosis $B[\rho^{(4)}]^{\text{(0)}} = B[\rho^{(4)}] - \bar{B}[\rho^{(4)}]$ and the fluctuation of the true PSF size, $\delta[\sigma_P] = \sigma_P - \bar{\sigma}_P$. The 2PCF of two quantities $y_1$ and $y_2$ is defined by
% \begin{equation}
% \xi(\theta) = \langle y_1(x) y_2(x+\theta) \rangle. 
% \end{equation}
% Here $y_1$ and $y_2$ can be the same parameters, when computing an auto-correlation function, or different ones, when computing cross-correlations. 
% The 2PCF is measured using \textsc{TreeCorr}\footnote{\url{https://github.com/rmjarvis/TreeCorr}} \citep{2004MNRAS.352..338J}. The statistical uncertainty in the 2PCF is measured using a jackknife, with $N_{\text{patch}} = 30$. 


%\subsection{Bias in cosmic shear}
% \label{sec:2pt_correlation_bias}


% Finally, we describe how we estimate the bias in weak lensing shear-shear correlation functions induced by the estimated level of higher moment error in the PSF.  For the simple case considered here, focusing on radial kurtosis bias, shear biases are purely multiplicative and the kurtosis residuals that generate them are independent of the weak lensing signal, we will now show that the bias on the weak lensing shear-shear correlation functions should be a  multiplicative bias as well. 


% For a given sample of galaxies used to measure the weak lensing shear, the shear field depends on the position on the sky $\mathbf{x}$; so does the kurtosis bias, and therefore the associatd shear multiplicative bias.  The observed shear $\hat{g}(\mathbf{x}) = [1+m(\mathbf{x})] g(\mathbf{x})$, where the $g(\mathbf{x})$ is the true shear.  When $|m| \ll 1$, the observed shear correlation function is
% \begin{equation}
%     \langle \hat{g}(\mathbf{x}) \hat{g}(\mathbf{x+\theta})\rangle = \langle [1+m(\mathbf{x})] g(\mathbf{x})[1+m(\mathbf{x+\theta})] g(\mathbf{x+\theta})\rangle.
% \end{equation}
% Since $m\ll 1$, we ignore the $m^2$ term and focus on the first order expansion:
% \begin{align}
%     \nonumber \langle \hat{g}(\mathbf{x}) \hat{g}(\mathbf{x+\theta})\rangle = & \langle  g(\mathbf{x}) g(\mathbf{x+\theta})\rangle + \langle m(\mathbf{x}) g(\mathbf{x}) g(\mathbf{x+\theta})\rangle\\
%     & +  \langle  m(\mathbf{x+\theta}) g(\mathbf{x}) g(\mathbf{x+\theta})\rangle.
% \end{align}
% To simplify the second and third terms, we rely on the fact that the kurtosis field and therefore the $m(\mathbf{x})$ field are generated by the physics of the PSF, which means they are independent of the cosmological shear field $g(\mathbf{x})$. For two independent random variables, the average of the product is the product of the average.  As a result, we conclude that
% \begin{align}
%     \nonumber\langle \hat{g}(\mathbf{x}) \hat{g}(\mathbf{x+\theta})\rangle = & \langle  g(\mathbf{x}) g(\mathbf{x+\theta})\rangle + \langle m(\mathbf{x})\rangle \langle g(\mathbf{x}) g(\mathbf{x+\theta})\rangle\\\nonumber
%     & +  \langle  m(\mathbf{x+\theta})\rangle \langle g(\mathbf{x}) g(\mathbf{x+\theta})\rangle\\
%      = & (1 + 2\langle m\rangle) \langle  g(\mathbf{x}) g(\mathbf{x+\theta})\rangle.
% \end{align}
% This means that the shear bias caused by the PSF radial kurtosis bias results in a multiplicative bias in the shear 2PCF, as well.  


% The mean multiplicative bias of a galaxy ensemble can be calculated by $\langle m \rangle = \langle (\partial m/ \partial B[\rho^{(4)}]) B[\rho^{(4)}] \rangle$, when there is no other source of systematics. \response{Since the shape and shear biases are proportional to the kurtosis bias, as we later find out, we can estimate the shear bias by taking the first term of Taylor expansion
% \begin{equation}
% \label{eq:m_estimate}
%     m(B[\rakurto]) \approx \frac{\partial m}{ \partial B[\rakurto]} B[\rakurto].
% \end{equation}
% }The first factor in the equation above is determined by the galaxy population and the second factor purely depends on the PSF, they are independent random variables and the averages can be separately calculated.
% As a result, for a galaxy ensemble, $\langle m \rangle = \langle \partial m/ \partial B[\rho^{(4)}] \rangle \langle B[\rho^{(4)}] \rangle $.  Functionally, this means that we can simply calculate the average of $ B[\rho^{(4)}] $ over the PSF model across the survey, and average $\partial m/ \partial B[\rho^{(4)}]$ over the galaxy population.  Those two separate results can be combined to estimate an average weak lensing shear bias for galaxy populations that resemble those that will be used for measurements of weak lensing in any survey such as LSST. 


%Since the PSF in this simulation has a single size and therefore galaxy size maps uniquely to a galaxy-to-PSF size ratio, this result agrees with the conclusions from the single galaxy experiments.  



%The two-point statistics of these maps and their cross-correlations with second moment $\sigma$ are shown in Appendix~\ref{ap:one_two_point_statistics}
    .



%\rachel{Look at MNRAS author guidelines (\url{https://academic.oup.com/mnras/pages/General_Instructions}) section 2.9 for more on required elements regarding data availability.}\tianqing{Add after the Acknowledgments}


%\rachel{MNRAS author guide specifies that appendices are to be located after references, so you should move all of this.}


%\rachel{There is an interesting feature that you haven't commented on: if the differences were purely due to noise, the model PSF kurtosis histogram would be broader than the true PSF kurtosis histogram, but in fact the opposite is true -- the true PSF kurtosis histogram is broader and extends to noticably lower kurtosis values.  This is certainly worth pointing out!}\tianqing{I don't think the width is caused by the noise, it is the actual spatial structure of the PSF true kurtosis. In other words, at a certain position, the width of both model and truth kurtosis is much smaller than this width.} \rachel{I agree that the width is not due to noise.  I am asking you to put yourself in the perspective of a random reader.  The nominal expectation is that (1) the width of the true PSF kurtosis histogram is due to survey observing conditions, and (2) if the PSF modeling process is perfect, the PSF model kurtosis histogram should be identical.  Deviations from this in basic quantities like average value or width can be naturally interpreted, the latter perhaps due to noise.  Right now you are presenting these histograms without any interpretation, and in cases like that, you should either ask yourself if the figure is perhaps unnecessary, or if you should add an interpretation.  I recommend the latter.}\done We find that the model PSF kurtosis is on average  







% \begin{figure*}
%     \centering
%     \includegraphics[width=1.5\columnwidth]{plots/hsc_correlation.pdf}
%     \caption{\label{fig:hsc_2pt}Auto- and cross-correlation functions between kurtosis fluctuation $\delta \rho^{(4)} (x)$, the zero-averaged kurtosis residual $\tilde{B}[\rakurto](x)$ and the fluctuation of the PSF size $\delta \sigma_P (x)$.  %\rachel{reconsider notation}\done . 
%     The errorbars on the correlation functions are generated using jackknife resampling with 30 patches.  %\rachel{main text says 30}\done. 
%     The orange vertical lines represent the angular diameter of the HSC field of view, 90$'$. %\rachel{Axis and ticktext is too small.}\done 
%     } 
% \end{figure*}


% Next, we calculate the two-point statistics between the kurtosis fluctuation $\delta \rakurto (x) =  \rakurto(x) - \langle \rakurto(x) \rangle $, the zero averaged fractional kurtosis bias $\tilde{B}[\rakurto](x) = B[\rakurto](x) - \langle B[\rakurto](x) \rangle$, defined in Eq~\eqref{eq:kurtosis_error} and the PSF size fluctuation $\delta \sigma_P (x) = \sigma_P (x) - \langle \sigma_P(x)\rangle$, shown in Fig.~\ref{fig:hsc_2pt}. The errorbars of the auto- and cross-correlations are generated using the jackknife method with 30 patches in the area. 
% The errorbars on the correlation function are significantly larger than the point-to-point fluctuations because they reflect coherent fluctuations across the HSC survey area induced by large-scale systematics. We can see that these quantities exhibit non-zero correlations that drop to zero on a scale of $100\arcmin$, comparable to the $90\arcmin$ FOV of HSC.  
% This result implies 
% that the PSF kurtosis bias may be related to  challenges in modeling the PSF components associated with variation on scales of the full focal plane (e.g., due to the telescope optics) rather than on smaller scales, e.g., chip-to-chip variations. 











































































